Knapsack with Vertex Cover, Set Cover, and Hitting Set

Given an undirected graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, with vertex weights $(w(u))_{u\in\mathcal{V}}$, vertex values $(\alpha(u))_{u\in\mathcal{V}}$, a knapsack size $s$, and a target value $d$, the \vcknapsack problem is to determine if there exists a subset $\mathcal{U}\subseteq\mathcal{V}$ of vertices such that $\mathcal{U}$ forms a vertex cover, $w(\mathcal{U})=\sum_{u\in\mathcal{U}} w(u) \le s$, and $\alpha(\mathcal{U})=\sum_{u\in\mathcal{U}} \alpha(u) \ge d$. In this paper, we closely study the \vcknapsack problem and its variations, such as \vcknapsackbudget, \minimalvcknapsack, and \minimumvcknapsack, for both general graphs and trees. We first prove that the \vcknapsack problem belongs to the complexity class \NPC and then study the complexity of the other variations. We generalize the problem to \setc and \hs versions and design polynomial time $H_g$-factor approximation algorithm for the \setckp problem and d-factor approximation algorithm for \hstp using primal dual method. We further show that \setcks and \hsmb are hard to approximate in polynomial time. Additionally, we develop a fixed parameter tractable algorithm running in time $8^{\mathcal{O}({\rm tw})}\cdot n\cdot {\sf min}\{s,d\}$ where ${\rm tw},s,d,n$ are respectively treewidth of the graph, the size of the knapsack, the target value of the knapsack, and the number of items for the \minimalvcknapsack problem.

==> main-old.tex <==
\begin{abstract}
In the \vcknapsack problem, we are given an undirected graph $\GG=(\VV,\EE)$, with vertex weights $(w(u))_{u\in\VV}$, vertex values $(\alpha(u))_{u\in\VV}$, a knapsack size $s$, and a target value $d$, and the goal is to compute if there exists a vertex cover $\UU\subseteq\VV$ with $w(\UU)=\sum_{u\in\UU} w(u) \le s$, and $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$. This problem simultaneously generalizes the classical vertex cover and knapsack problems. We show that the problem is strongly \NPC. However, it admits a pseudo-polynomial time algorithm for trees. In fact, we show that there is an algorithm which runs in time $\OO\left(2^{\OO(\tw)}\cdot n\cdot {\sf min}\{s^2,d^2\}\right)$. {\color{red} Write the $(1-\eps)$ approximation algorithm...} We then consider polynomial-time algorithms and present a $2$ factor polynomial-time approximation algorithm for this problem for minimizing the total weight of the solution. On the other hand, we show that there is no $\rho$ factor polynomial-time approximation algorithm for maximizing the total value of the solution given a knapsack size for any $\rho>1$ unless $\Pb=\NP$.

We study the above problem when the solution \UU needs to be a minimal vertex cover, minimum vertex cover, vertex cover of size at most $k$ for some input integer $k$ and show similar results. Then, we consider set families (equivalently hypergraphs) and study the above problem when the solution needs to be a set cover and hitting set. We show that there are $H_g$ and $f$ factor polynomial-time approximation algorithms for \setck for minimizing the weight of the knapsack given a target value and a $d$ factor polynomial-time approximation algorithm for \hstp. On the other hand, we show that there is no $\rho$ factor polynomial-time approximation algorithm for maximizing the total value of the solution given a knapsack size for any $\rho>1$ unless $\Pb=\NP$ for both \setck and \hstp.

% In this paper, we closely study the \vcknapsack problem and its variations, such as \vcknapsackbudget, \minimalvcknapsack, and \minimumvcknapsack, for both general graphs and trees. We first prove that the \vcknapsack problem belongs to the complexity class \NPC and then study the complexity of the other variations. We generalize the problem to \setc and \hs versions and design polynomial time $H_g$-factor approximation algorithm for the \setckp problem and d-factor approximation algorithm for \hstp using primal dual method. We further show that \setcks and \hsmb are hard to approximate in polynomial time. Additionally, we develop a fixed parameter tractable algorithm running in time $8^{\tw + 1}\cdot n\cdot {\sf min}\{s^2,d^2\}$  where $\tw,s,d,n$ are respectively treewidth of the graph, the size of the knapsack, the target value of the knapsack, and the number of items for the \minimalvcknapsack problem. 
\end{abstract}

\section{Introduction}
\label{sec:introduction}

The \vc problem is a well-studied classical problem in graph theory and operations research. Given a graph $\GG(\VV, \EE)$, the \vc problem aims to find a minimum vertex subset $\VV^\pr \subseteq \VV$ such that for every edge $(u,v) \in \GG[\EE]$, either $u$ or $v$ or both exist in $\VV^\pr$. In this paper, we explore a novel variation of the classical \vc problem in the context of the \kp. In the \kp problem, we are given a set of $n$ items, \XX = \{1, 2, \dots, n\} and a knapsack of capacity $b$. Each item $i \in [n]$ is associated with size $\theta_i$ and values $p_i$. The computational question is to find a subset $\II \subseteq \XX$ to be put into the knapsack of capacity $b$ that maximizes the value of the knapsack without exceeding its capacity constraint. This paper delves into the problem \vcknapsack, where given an undirected graph $\GG=(\VV,\EE)$, with vertex weights $(w(u)){u\in\VV}$, vertex values $(\alpha(u)){u\in\VV}$, a knapsack size $s$, and a target value $d$, the \vcknapsack problem is to determine if there exists a subset $\UU\subseteq\VV$ of vertices such that \UU forms a vertex cover, $w(\UU)=\sum_{u\in\UU} w(u) \le s$, and $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$. We study several interesting variations of this problem like \vcknapsackbudget, \minimalvcknapsack, and \minimumvcknapsack. These problems are formally defined in Section \ref{pd}. \vc is a special case of \setc and 2-HITTING SET. We design polynomial time approximation algorithms for \setckp problem and show similar results for \hs and \vcknapsack. We also show that \vckmb does not admit a polynomial time approximation algorithm unless $P = \NP$.

These problems often find applications in various domains, including wireless network design, especially in the context of leasing mobile towers. Consider a scenario where a company aims to establish mobile towers in different areas to efficiently serve its customers while minimizing leasing costs within a budget constraint. Additionally, the company must ensure that it meets the target or subscribed customer base. This situation can be depicted through an undirected weighted graph \GG, where vertices symbolize towers and edges represent the connectivity range. Each tower vertex is associated with a value, indicating the number of customers it can serve, and a weight, representing the leasing cost. Moreover, there exists a budget constraint, limiting the total cost the company can afford for leasing towers, alongside a target value representing the desired total value in terms of the number of customers served.

In the subsequent sections, we first present a brief overview of the efforts made in the realm of the \vc problem in Section \ref{related}. We formally define the problems in Section \ref{pd}. We show the classical NP Completeness results in Section \ref{npcresults}. We develop polynomial time approximation algorithms and a fixed parameter tractable algorithm in Section \ref{approximation} and Section \ref{parameterized} respectively. We conclude our efforts in Section \ref{conclusion}.


\subsection{Contributions}
We study the computational complexity of the problems \vcknapsack, \vcknapsackbudget, \minimumvcknapsack, and \minimalvcknapsack. For each of these problems, we resolve their complexity with respect to general graphs and trees. We design a polynomial time 2-approximation algorithm for the problem using primal dual method. Further we also demonstrate that the \vcknapsack, \minimumvcknapsack and \minimalvcknapsack all admit fixed parameter tractable algorithms with \textit{treewidth} as the parameter. 
Our main contributions are highlighted in Table \ref{tab:contribution}.

\begin{table}
	\centering 
	\begin{tabular}{|c|c|}\hline
		\vcknapsack & \makecell{strongly \NPC (Theorem \ref{thm:vckp-gen-npc})\\pseudo-polynomial for trees (Corollary \ref{thm:vckp-tree-algo}) \\ $2^{\OO(\tw)}\cdot n\cdot {\sf min}\{s^2,d^2\}$ (Theorem \ref{vckparameterzied})} \\\hline
        
		\vcknapsackbudget & \makecell{strongly \NPC (Theorem \ref{thm:vckb-gen-npc})\\pseudo-polynomial for trees (Corollary \ref{tree-pseudo-poly}) \\ $\OO(n^2\cdot min\{s^2, (\alpha(\VV))^2\})$ (Corollary \ref{tree-pseudo-poly})} \\\hline
  
		\minimumvcknapsack & \makecell{\NP hard (Observation \ref{obs:minvckp-not-poly}) \\\NPC for trees \\ $4^{\OO(\tw)}\cdot n\cdot {\sf min}\{s^2,d^2\}$ (Theorem \ref{minvckparameterzied}) }\\\hline
  
		\minimalvcknapsack & \makecell{strongly \NPC (Theorem \ref{thm:minimalvckp-gen-npc}) \\\NPC for trees (Theorem \ref{minimalvck-trees-npc})\\ no poly-time approx. algorithm (Theorem \ref{minimalvcknapssackhoa})\\ $8^{\tw + 1}\cdot n\cdot {\sf min}\{s^2,d^2\}$ (Theorem \ref{fptminimal})}\\\hline

         \setckp & \makecell{poly-time f-approx. algorithm (Theorem \ref{thm:approxf})\\  poly-time $ H_g$-approx algorithm (Theorem \ref{hgapprosetcover})} \\ \hline

         \setcks & \makecell{no poly-time approx. algorithm (Theorem \ref{hardnessofapprox}) } \\ \hline

        
        \hstp & \makecell{poly-time d-approx. algorithm (Corollary \ref{hsdfactor})} \\ \hline
        
        \hsmb & \makecell{no poly-time approx. algorithm (Corollary \ref{hoa:dhs})} \\ \hline

         \vcktp & \makecell{poly-time 2-approx. algorithm (Corollary \ref{2factorvc})} \\ \hline

        \vckmb & \makecell{no poly-time approx. algorithm (Corollary \ref{vc-no-poly-approx})} \\ \hline

        
	\end{tabular}
	\caption{Summary of results}
	\label{tab:contribution}
\end{table}




\subsection{Related Work}
\label{related}
\vc is a well-studied \NPC problem in Graph Theory. Given a graph \GG = (\VV, \EE), a vertex cover for G is any subset $\VV^\pr \subseteq \VV$ that contains at least one endpoint from every edge. The problem is also investigated to be \NPC in planar graphs with a degree at most 3 \cite{garey1977rectilinear}\cite{garey1979computers}. \textit{Weighted} \vc (WVC) is the weighted version studied in different literature where the sum of weights of all the vertices in a \vc must be $\leq c$ (where $c \in \mathbb{R^+}$). If all the weights of the vertices are $1$, it is called \textit{Unweighted} \vc (UVC). In the paper~\cite{niedermeier2003efficient}, Niedermeier and Rossmanith proved that WVC is \textit{fixed-parameter tractable} if the weights are positive integers or real numbers $\geq 1$, but it is \textit{not} fixed-parameter tractable if the weights are positive real numbers unless $\textbf{P}=\NP$. They used a dynamic programming algorithm with complexity $\OO((1.3788)^c + cn)$, where $n$ is the number of vertices of the input graph. Later, Fomin et al~\cite{fomin2006branching} provided an algorithm to improve the running time to $\OO((1.357)^c \cdot n)$ . Chlebíka and Chlebíková~\cite{chlebik2008crown} proposed an exact algorithm by using the crown reduction technique for solving the Minimum Weighted Vertex Cover (MWVC) problem, whose decision version is WVC. Approximation algorithms for MWVC are described here~\cite{ausiello2012complexity}. Linear time 2-approximation algorithms exist for both UVC~\cite{vazirani2001approximation} and WVC~\cite{bar1981linear}. These results become improved with a better approximation factor for UVC~\cite{monien1985ramsey} and WVC~\cite{bar1985local}

k-\vc (the decision version of the Minimum \vc problem) finds a vertex cover of size at most $k$ (where $k \in \mathbb{Z^+}$) or returns that no such size of \vc exists. This problem is \FPT. The first \FPT algorithm for this problem with a time complexity of $\OO(2^k\cdot n)$ was given by Downey and Fellows~\cite{downey2012parameterized}. They used the technique of bounded search trees. S. Buss~\cite{downey2012parameterized} proved that this problem is solvable in $\OO(k^k + n)$ time. The algorithm developed by Papadimitriou and Yannakakis~\cite{stege1999improved} has a running time of $\OO(3^k\cdot n)$. In the paper~\cite{balasubramanian1998improved}, Balasubramanian et al. gave an algorithm with a running time of $\OO((1.324718)^k\cdot k^2 + kn)$ using bounded search techniques. Downey et al.\cite{downey1997parameterized} developed an algorithm using kernelization and search tree methods with a complexity of $\OO((1.31951)^k\cdot k^2 + kn)$. Later, Niedermeier and Rossmanith\cite{niedermeier1999upper} provided an algorithm with complexity $\OO((1.29175)^k \cdot k^2 + kn)$. Another \FPT algorithm with a running time of $\OO(\max{(1.25542)^k \cdot k^2, (1.2906)^k\cdot k} + kn)$ was given by Stege and Fellows~\cite{fellows1999improved}. The best-known result, provided by Harris and Narayanaswamy~\cite{DBLP:conf/stacs/0001N24}, gives an algorithmic complexity of $\OO((1.25284)^k + kn)$.

  


\maxminimalvc (MMVC) is a problem of finding a minimal \vc of cardinality at least $k$. This problem admits a polynomial kernel in terms of the number of vertices and can be solved in $\OO(2^k+p(n))$ time using a search tree algorithm, where $p$ is some polynomial~\cite{fernau2005parameterized}. Later, Peter Damaschke~\cite{damaschke2011parameterized} proved that MMVC is solvable in time $\OO^(1.62^k)$. For general graphs, Boria et al~\cite{boria2015max} showed that this problem is polynomially approximable within the ratio $n^{-1/2}$ and inapproximable within the ratio $n^{\epsilon-1/2}$ unless $\textbf{P}=\NP$, where $\epsilon > 0$. They proved that this problem is \FPT and can be solved in $\OO^(1.5739^{opt})$ with respect to the cardinality of the optimal solution ($opt$), in $\OO^*(2.8284^{M})$ with respect to the size of the maximum matching ($M$), and also with respect to the treewidth.


Various approximation algorithms have been explored for the \setc problem like $f$ factor, $\log n$ and $\log d$, factor approximation ratios \cite{williamson2011design}. Here $n$ and $d$  denote the number of elements in the universe and frequency of the most frequent element respectively. Delbot and  Laforest in \cite{delbot2010analytical} concluded that we cannot hope to have an approximation algorithm for vertex cover better than 2.

There are several other variations of the classical \vc problem studied in the literature, such as \textit{Connected} \vc in ~\cite{li2019connected}, \cite{escoffier2010complexity}, and \textit{Eternal Connected} \vc in \cite{paul2024eternal}, \cite{fujito2020eternal}. In this study, we explore a novel variant of the \vc problem, namely \vcknapsack. Given an undirected weighted graph \GG, the size of the knapsack, and a target value, the computational question is to compute a vertex cover that yields the maximum profit without exceeding the size of the knapsack. We formally define the problem in Section \ref{pd}. Our main results prove that this problem is \NPC.


\section{Preliminaries}
\label{pd}

This section is devoted to formally define the \vcknapsack problem and its variants. In the \vcknapsack problem, we are given an undirected graph $\GG=(\VV,\EE)$, where each vertex is associated with a non-negative weight, $(w(u))_{u\in\VV}$ and non-negative value, $(\alpha(u))_{u\in\VV}$. We are also given a knapsack of size $s$ and target value $d$. We want to obtain a vertex cover, $\UU \subseteq \VV$ that additionally satisfies the knapsack constraints i.e. the weight of all the vertices in \UU, denoted by $w(\UU)=\sum_{u\in\UU} w(u)$,  must be at most the size of the knapsack, $s$ and the value of all the vertices in \UU, denoted by $\alpha(\UU)=\sum_{u\in\UU} \alpha(u)$ must be at least $d$.
\begin{definition}[\vcknapsack]\label{vckp}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, size $s$ of knapsack, and target value $d$, compute if there exists a subset $\UU\subseteq\VV$ of vertices such that:
	\begin{enumerate}
		\item \UU is a vertex cover.
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
	We denote an arbitrary instance of \vcknapsack by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$.
\end{definition}

To the \vcknapsack problem defined above, we add another constraint by restricting the number of vertices in \UU i.e. the size of the vertex cover can be at most k ($|\UU| \leq k$). We call this problem as \vcknapsackbudget. \shortversion{We denote an arbitrary instance of \vcknapsackbudget by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d,k)$.}
\longversion{\begin{definition}[\vcknapsackbudget]\label{vckpb}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, budget $k$ of the vertex cover, size $s$ of knapsack, and target value $d$, compute if there exists a subset $\UU\subseteq\VV$ of vertices such that:
	\begin{enumerate}
		\item \UU is a \vc of size at most $k$,
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
	We denote an arbitrary instance of \vcknapsackbudget by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d,k)$.
\end{definition}}
Similarly, as another variant of \vcknapsack we want the vertex cover \UU to be a minimum vertex cover. We call this version as \minimumvcknapsack. \shortversion{We denote an arbitrary instance of \minimumvcknapsack by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$.}
\longversion{\begin{definition}[\minimumvcknapsack]\label{minimumvckp}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, size $s$ of knapsack, and target value $d$, compute if there exists a subset $\UU\subseteq\VV$ of vertices such that:
	\begin{enumerate}
		\item \UU is minimum \vc,
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
	We denote an arbitrary instance of \minimumvcknapsack by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$.
\end{definition}}
 We also explore another interesting version of the \vcknapsack problem where we desire the vertex cover \UU to be a minimal vertex cover. We name this problem as \minimalvcknapsack. \shortversion{We denote an arbitrary instance of \minimalvcknapsack by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$.}
\longversion{\begin{definition}[\minimalvcknapsack]\label{minimalvckp}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, size $s$ of knapsack, and target value $d$, compute if there exists a subset $\UU\subseteq\VV$ of vertices such that:
	\begin{enumerate}
		\item \UU is a minimal \vc,
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
	We denote an arbitrary instance of \minimalvcknapsack by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$.
\end{definition}}

\begin{definition}[\twd] 
Let $G = (V_G,E_G)$ be a graph.  A \textit{tree-decomposition} of a graph $G$ is a pair 
$(\mathbb{T} = ((V_{\mathbb{T}},E_{\mathbb{T}}),\mathcal{ X}=\{X_{t}\}_{t\in V_{\mathbb{ T}}})$,  where 
${\mathbb{ T}}$ is a tree where every node $t\in V_{\mathbb{ T}}$ 
is assigned a subset $X_t\subseteq V_G$, called a bag,  such that the following conditions hold. 
\begin{itemize}
%\setlength{\itemsep}{-2pt}
\item $\bigcup_{t\in V_\mathbb{T}}{X_t}=V_G$,
\item for every edge $\{x,y\}\in E_G$ there is a $t\in V_\mathbb{T}$ such that  $x,y\in X_{t}$, and 
\item for any $v\in V_G$ the subgraph of $\mathbb{T}$ induced by the set  $\{t\mid v\in X_{t}\}$ is connected.
\end{itemize}
\end{definition}
The \textit{width} of a tree decomposition is $\max_{t\in V_\mathbb{T}} |X_t| -1$. The \textit{treewidth} of $G$ 
is the  minimum width over all tree decompositions of $G$ and is denoted by $\tw(G)$. 
 
A tree decomposition  $(\mathbb{T},\mathcal{ X})$ is called a \textit{nice edge tree decomposition} if $\mathbb{T}$ is a tree rooted at some node $r$ where $ X_{r}=\emptyset$, each node of $\mathbb{T}$ has at most two children, and each node is of one of the following kinds:
\begin{itemize}
%%%\setlength\itemsep{-1mm}
%\setlength{\itemsep}{-2pt}
\item {\bf Introduce node}: a node $t$ that has only one child $t'$ where $X_{t}\supset X_{t'}$ and  $|X_{t}|=|X_{t'}|+1$.
\item {\bf  Forget vertex node}: a node $t$ that has only one child $t'$  where $X_{t}\subset X_{t'}$ and  $|X_{t}|=|X_{t'}|-1$.
\item {\bf Join node}:  a node  $t$ with two children $t_{1}$ and $t_{2}$ such that $X_{t}=X_{t_{1}}=X_{t_{2}}$.
\item {\bf Leaf node}: a node $t$ that is a leaf of $\mathbb T$, and $X_{t}=\emptyset$. 
\end{itemize}
We additionally require that every edge is introduced exactly once. 
One can  show that  a tree decomposition of width $t$ can be transformed into 
a nice tree decomposition of the same width $t$ and  with 
 $\mathcal{O}(t |V_G|)$ nodes \cite{cygan2015parameterized}. For a node $t \in \mathbb{T}$, let $\mathbb{T}_t$ be the subtree of $\mathbb{T}$ rooted at $t$, and $V(\mathbb{T}_t)$ denote the vertex set in that subtree. Then $G_t$ is the subgraph of $G$ where the vertex set is  $\bigcup_{t' \in V(\mathbb{T}_t)} X_{t'}$ and the edge set is the union of the set of edges introduced in each $t', t' \in V(\mathbb{T}_t)$. We denote by $V(G_t)$ the set of vertices in that subgraph, and by $E(G_E)$ the set of edges of the subgraph.: a node $t$ that is a leaf of $\mathbb T$, and $X_{t}=\emptyset$. 

 In this paper, we sometimes fix a vertex $v\in V_G$ and include it in every bag of a nice edge tree decomposition $(\mathbb{T},\mathcal{X})$ of $G$, with the effect of the root bag and each leaf bag containing $v$. For the sake of brevity, we also call such a modified tree decomposition a nice tree decomposition. Given the tree $\mathbb{T}$ rooted at the node $r$, for any nodes $t_1,t_2 \in V_\mathbb{T}$, the distance between the two nodes in $\mathbb{T}$ is denoted by $\sf{dist}_\mathbb{T}(t_1,t_2)$.


%************************************************************************************************************************************************************************


\section{Results: Classical NP Completeness}
\label{npcresults}

%\section{\vcknapsack}\label{sec:res3a}
%\subsection{Hardness Results}
\begin{definition}[\vc]\label{vc}
	Given a graph $\GG=(\VV,\EE)$ and a positive integer $k$, compute if there exists a subset $\VV' \subseteq \VV$ such that at least one end-point of every edge belongs to $\VV'$ and $|\VV'|\leq k$. We denote an arbitrary instance of \vc by $(\GG,k)$.
\end{definition}

In this section, we show that \vcknapsack is strongly \NPC by reducing it from \vc(see, \cref{vc}).

\begin{theorem}\label{thm:vckp-gen-npc}
	\vcknapsack is strongly \NPC for general graph.
\end{theorem}

\begin{proof}
	Clearly, \vcknapsack $\in$ \NP. We reduce \vc to \vcknapsack to prove NP-hardness. Let $(\GG(\VV=\{v_i: i\in[n]\},\EE),k)$ be an arbitrary instance of \vc of size $k$. We construct the following instance $(\GG^\pr(\VV^\pr=\{u_i: i\in[n]\},\EE^\pr),(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d)$ of \vcknapsack.
	\begin{align*}
		&\VV^\pr = \{u_i : v_i\in \VV, \forall i\in[n]\}\\
		&\EE^\pr = \{\{u_i,u_j\}: \{v_i, v_j\} \in\EE, i\neq j, \forall i, j\in[n]\}\\
		&w(u_i) = 1, \alpha(u_i)=1 \qquad \forall i\in[n]\\
		&s =d = k
	\end{align*}
	The \vcknapsack problem has a solution iff \vc has a solution.\\
	
	\noindent
	Let $(\GG^\pr,(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d)$ of \vcknapsack such that $\WW^\pr$ be the resulting subset of $\VV^\pr$ with (i) $\WW^\pr$ is a \vc, (ii) $\sum_{u\in \WW^\pr} w(u) = k$, (iii) $\sum_{u\in \WW^\pr} \alpha(u) = k$\\
	\noindent
	This means that the set $\WW^\pr$ is a \vc which gives the maximum profit $k$ for the bag capacity of size $k$. In other words, $\WW^\pr$ is a \vc of size $k$. Since $\WW' =\{u_i: v_i \in \WW, \forall i \in[n]\}$, $\WW$ is a \vc of size $k$. Therefore, the \vc instance is an \yes instance.\\
	
	\noindent
	Conversely, let us assume that \vc instance $(\GG,k)$ is an \yes instance.\\ 
	Then there exists a subset $\WW\subseteq \VV$  of size $k$ such that it outputs a \vc. \\	
	\noindent
	Consider the set $\WW^\pr=\{u_i: v_i \in \WW, \forall i \in[n]\}$.
	Since each vertex of $\WW^\pr$ is involved with weight 1 and produces profit amount 1, $\WW^\pr$ is a \vc of max bag size and total profit $k$. 
	\noindent
	Therefore, the \vcknapsack instance is an \yes instance.\\
\end{proof}




\begin{comment}
\begin{theorem}\label{thm:vckp-tree-algo}
	There is an algorithm of \vcknapsack with complexity $\OO(n\cdot min\{s, (\alpha(\VV))\})$.
\end{theorem}
\begin{proof}
Let $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$ be an arbitrary instance of \vcknapsack. We develop a dynamic programming algorithm to compute \vcknapsack for trees \TT. Let \GG=\TT. This algorithm executes by computing the set of undominated weight-profit pairs of vertices of all Vertex Covers in $D[u,d_u]$ (including $u$) and $D[\bar{u},d_u]$ (without including $u$) for the vertex $u$ as the root of the tree \TT recursively from its next-level children $v_1, v_2,\ldots,v_{d_u}$. We Formally define $D[u,d_u]=\{(w_c,\alpha_c):\exists$ some $\vc$ $\CC$ with $w(\CC)=w_c<w(\CC')$ and/or $\alpha(\CC)=\alpha_c>\alpha(\CC')$, where $\CC'$ is another \vc and $u$ is included in both $\CC$ and $ \CC'\}$. $D[\bar{u},d_u]$ also carries the same definition but without including $u$. We consider the maximum degree of $u$ is $d_u$ and  $v_1, v_2,\ldots,v_{d_u}$ with maximum degree $d_{v_1},d_{v_2},\ldots,d_{v_{d_u}}$ respectively. After computing $D[u,d_u]$ and $D[\bar{u}, d_u]$, we remove dominated and duplicated weight-profit pairs from $D[u, d_u] \cup D[\bar{u}, d_u]$ and check the condition of the knapsack size $s$ so that the knapsack can contain each undominated weight-profit pair of \vc individually. So, output \YES if a pair exists $(w_c,\alpha_c) \in D[u, d_u] \cup D[\bar{u}, d_u]$ such that $w_c \leq s$ and $\alpha_c \geq d$ \\

\noindent
\textbf{Initialization:}  $D[u, 0]=\{(w(u),\alpha(u))\}, D[\bar{u}, 0]=\{(0,0)\}$ if $u$ is a leaf node.\\
%Otherwise $D[u,0]=\{(w(u),\alpha(u))\}$ and $D[\bar{u},0]=\{(0,0)\}$\\
\parindent=0cm 
\textbf{Updating DP table:} Suppose using bottom up recursive computation we have  $D[v_i,d_{v_i}]$ and $D[\bar{v_j},d_{v_j}]$ for each child $v_i$ of $u$. In $0^{th}$ iteration for $u$ we initialize $D[u,0]=\{(w(u),\alpha(u))\}$. Now for updation of $D[u,j]$ in $j^{th}$ iteration, initially we set $D[u,j]=\emptyset$ and update $D[u,j]$ to $D[u,j]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$ for each pair $(w_1, \alpha_1) \in D[v_j,d_{v_j}]\cup D[\bar{v_j},d_{v_j}]$ and each pair $(w_2, \alpha_2) \in D[u,j-1]$. Then, we remove dominated and duplicated pairs from $D[u,j]$. This process executes for each value of $j=1$ to $d_u$. And finally we get $D[u,d_u]$.\\
Similarly, for computing $D[\bar{u},d_u]$ we initialize $D[\bar{u},0]=\{(0,0)\}$ for $0^{th}$ iteration. Then first we set $D[\bar{u},j]=\emptyset$ and update $D[\bar{u},j]$ to $ D[\bar{u},j]\cup\{(w_3+w_4,\alpha_3+\alpha_4)\}$ for each pair $(w_3, \alpha_3) \in D[v_j,d_{v_j}]$ and each pair $(w_4, \alpha_4) \in D[\bar{u},j-1]$ for all $j=1$ to $d_u$. For finding $D[\bar{u},d_u]$, since $u$ is not a part of the Vertex Cover, so we consider all children of $u$ in \vc set.\\
\begin{figure}[H]
	\centering
	\includegraphics[height=4cm,width=6cm]{t1.pdf}
	\caption{ Sub-trees for the tree rooted at $u$ and the children of $u$ (used in \Cref{thm:vckp-tree-algo} and \Cref{thm:vckp_budget_trees-algo})}
	\label{fig:t1}
\end{figure}
\noindent
\textbf{Correctness:} After removal of all dominated and duplicated pairs from $D[u, d_u] \cup D[\bar{u}, d_u]$ such that $w_c \leq s$ and $\alpha_c \geq d$, we get the final set $\FF$ of undominated weight-profit pair of Vertex Covers. Now we will prove that each pair $(w_c,\alpha_c) \in \FF$, is a \vc $\CC$ such that $w(\CC)=w_c$ and $\alpha(\CC)=\alpha_c$. Let us consider $\exists$ an arbitrary pair $(w_c,\alpha_c) \in \FF$. In the above algorithm, we store $ (w(v),\alpha(v))$ in $D[v,0]$ if $v$ is leaf node. Since no vertex other than leaves is encountered in $0^{th}$ level, the above hypothesis holds trivially. Let us suppose $v_j$ is a non-leaf node, and it is the $j^{th}$ child of the root node $u$ and for all $j= 1$ to $d_u$, $D[v_j, d_{v_j}] \cup D[\bar{v_j},d_{v_j}]$ gives the sets of undominated weight-profit pair of Vertex Covers at (root-level -1). Now for the root node $u$, we compute $D[u, d_u]$ and  $D[\bar{u}, d_u]$. From the above algorithm, each pair $(w_1, \alpha_1) \in D[v_j,d_{v_j}]\cup D[\bar{v_j},d_{v_j}]$ is \vc. Moreover, each pair $(w_2, \alpha_2) \in D[u,j-1]$ have calculated from $0^{th}$ to $(j-1)^{th}$ subtree of $u$ ($v_1$ to $v_{j-1}$ including $u$), so $(w_2, \alpha_2)$ also be a vertex cover as for trees there is no overlapping of two subtrees. Since we are summing up the pairs $(w_1+w_2,\alpha_1+\alpha_2)$ and storing in $D[u,d_u]$, hence no pairs come twice in $D[u, d_u]$ and gives us \vc $\CC$ with $w(\CC)=w_c$ and $\alpha(\CC)=\alpha_c$ for some arbitrary pair $(w_c,\alpha_c)$. When we consider $D[\bar{u},d_u]$, it is more clear to say that every pair is a \vc because $D[v_j, d_{v_j}]$  gives the sets of undominated weight-profit pair of Vertex Covers for all $j= 1$ to $d_u$. Thus, by considering the hypothesis TRUE in (root -1)$^{th}$ level, we proved by induction that it is also TRUE for the root node. \\

\noindent
\textbf{Complexity:} For each $n$ vertices we are computing $D[u,d_{u}]$ and $D[\bar{u},d_{u}]$ for all $u \in \VV$. In computation of $D[u,d_{u}]$ we store $D[u,j]$ to $D[u,j]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$ for each pair $(w_1, \alpha_1) \in D[v_j,d_{v_j}]\cup D[\bar{v_j},d_{v_j}]$ and each pair $(w_2, \alpha_2) \in D[u,j-1]$. So, this part gives the complexity $\OO( min\{s^2, (\alpha(\VV))^2\})$ as each table entry can contain at most $min\{s, (\alpha(\VV))\}$ pairs and similarly for  $D[\bar{u},d_{u}]$. Hence the total complexity is $\OO(n\cdot min\{s^2, (\alpha(\VV))^2\})$.



\end{proof}
\end{comment}


\begin{comment}
	
\subsection{Algorithmic Results}
\subsubsection{Algorithm}\label{sec:algo_dp_vc_trees}

We compute $D[u,d_u]$ and $D[\bar{u},d_u]$ from $D[v_1,d_{v_1}]$, $D[\bar{v_1},d_{v_1}]$, $D[v_2,d_{v_2}]$, $D[\bar{v_2},d_{v_2}] \ldots D[v_k,d_{v_k}]$, $D[\bar{v_k},d_{v_k}]$, where $D[u,d_u]$ is the set of weight-profit pairs of vertices including $u$ and $D[\bar{u},d_u]$ also carries the same meaning but without including $u$. We consider $u$ with the maximum degree $d_u(=k)$ as the root of the tree \TT  and  $v_1, v_2,\ldots,v_k$ are the next-level children of $u$ with maximum degree $d_{v_1},d_{v_2},\ldots,d_{v_k}$ respectively.\\


%\textbf{$D(u, d_u)$}
%\vcknapsack($\TT,u, d_u$)

\textbf{COMPUTE} D[$u, d_u$]
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		%\State $\textbf{T(u,d_u)}$
		\If{$u$ is a leaf node}
		\State $D[u,0]\leftarrow \{(w(u),\alpha(u))\}$;
		\State \textbf{return} $D[u,0]$;
		\Else
		%\State\textcolor{red}{ $Temp\leftarrow\emptyset$;}
		\State $D[u,0]\leftarrow\{(w(u),\alpha(u))\}$
		
		%\For{ $i=1$ to $k$}
		\For{$j=1$ to $d_u$}
		%\State\textcolor{red}{ $D[u,j]\leftarrow D[u,j-1]$;}
		\State $D[u,j]\leftarrow\emptyset$;
		
		\State \textbf{COMPUTE} D[$v_j, d_{v_j}$];
		\State \textbf{COMPUTE} D[$\bar{v_j}, d_{v_j}$];
		
		%\State \call {$\vcknapsack(\TT,v_j, d_{v_j})$};
		\For{each pair $(w_1, \alpha_1) \in D[v_j,d_{v_j}]\cup D[\bar{v_j},d_{v_j}]$}
		\For{each pair $(w_2, \alpha_2) \in D[u,j-1]$}
		%\State 			\textcolor{red}{$Temp\leftarrow Temp\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$;}
		\State$D[u,j]\leftarrow D[u,j]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$;
		
		
		\EndFor
		\EndFor
		
		%\State \textcolor{red}{$D[u,j]\leftarrow Temp$;}
		%\State \textcolor{red}{$Temp\leftarrow\emptyset$;}
		\State Remove dominated and duplicate pairs from $D[u,j]$;
		\EndFor
		\State \textbf{return} $D[u,d_u]$;
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}
%\end{Algorithms}
The function \textbf{COMPUTE} D[$u, d_u$] returns all undominated weight-profit pairs, which are individually a solution of a \vc that must include $u$ for the given tree $\TT$ where $u\in \VV$ and $d_u$ is the max degree of $u$. Lines 1 to 3 execute if $u$ is a leaf node; otherwise, lines 4 to 18 execute. In lines 6 to 16 \textbf{COMPUTE} D[] function executes recursively to find undominated \vc pairs for each of the child of $u$.

\textbf{COMPUTE} D[$\bar{u}, d_u$]
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		%\State $\textbf{T(u,d_u)}$
		\If{$u$ is a leaf node}
		\State $D[\bar{u},0]\leftarrow \{(0,0)\}$;
		\State \textbf{return} $D[\bar{u},0]$;
		
		\Else
		
		\State $D[\bar{u},0]\leftarrow\{(0,0)\}$
		\For{$j=1$ to $d_u$}
		\State $D[\bar{u},j]\leftarrow\emptyset$;
		
		%\State \textbf{COMPUTE} D[$v_j, d_{v_j}$];
		%\State \textbf{COMPUTE} D[$\bar{v_j}, d_{v_j}$];
		
		%\State \call {$\vcknapsack(\TT,v_j, d_{v_j})$};
		\For{each pair $(w_3, \alpha_3) \in D[v_j,d_{v_j}]$}
		\For{each pair $(w_4, \alpha_4) \in D[\bar{u},j-1]$}
		
		\State$D[\bar{u},j]\leftarrow D[\bar{u},j]\cup\{(w_3+w_4,\alpha_3+\alpha_4)\}$;
		
		\EndFor
		\EndFor
		
		\State Remove dominated and duplicate pairs from $D[\bar{u},j]$;
		\EndFor
		\State \textbf{return} $D[\bar{u},d_u]$;
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}
%\end{Algorithms}
%\parskip 2em
Similarly, \textbf{COMPUTE} D[$\bar{u}, d_u$] returns the solution pairs of \vc that must not include $u$.\\

\textbf{VCKnapsack}($\TT, s, u, d_u$)
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		
		\State \textbf{COMPUTE} D[$u, d_u$];
		\State \textbf{COMPUTE} D[$\bar{u}, d_u$];
		\State Remove dominated and duplicate weight-profit pairs from $D[u, d_u] \cup D[\bar{u}, d_u]$ such that each weight $\leq s$;
		\State \textbf{return} $D[u, d_u] \cup D[\bar{u}, d_u]$;
	\end{algorithmic}
\end{breakablealgorithm}
The function \textbf{VCKnapsack} calls the two recursive functions in lines 1 and 2. After getting the two undominated solution pair sets again, we remove the dominating pairs from $D[u, d_u] \cup D[\bar{u}, d_u]$ and we check the condition of the knapsack size $s$ so that the knapsack can contain them individually. Finally, we get our desired solution in line 4.
\end{comment}




%\break
\subsection{\vcknapsackbudget}\label{sec:res3b}

In this section, we show that \vcknapsackbudget is strongly \NPC by reducing it from \vc(see, definition \ref{vc}).

\begin{theorem}\label{thm:vckb-gen-npc}
	\vcknapsackbudget is strongly \NPC for general graph.
\end{theorem}

\begin{proof}
	Clearly, \vcknapsackbudget $\in$ \NP. We reduce \vc to \vcknapsackbudget to prove NP-hardness. Let $(\GG(\VV=\{v_i: i\in[n]\},\EE),k)$ be an arbitrary instance of \vc of size $k$. We construct the following instance $(\GG^\pr(\VV^\pr=\{u_i: i\in[n]\},\EE^\pr),(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d,k')$ of \vcknapsackbudget.
	\begin{align*}
		&\VV^\pr = \{u_i : v_i\in \VV, \forall i\in[n]\}\\
		&\EE^\pr = \{\{u_i,u_j\}: \{v_i, v_j\} \in\EE, i\neq j, \forall i, j\in[n]\}\\
		&w(u_i) = 1, \alpha(u_i)=1 \qquad \forall i\in[n]\\
		&s =d = k'=k
	\end{align*}
	The \vcknapsackbudget problem has a solution iff \vc has a solution.\\
	Let $(\GG^\pr(\VV^\pr,\EE^\pr),(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d,k')$ of \vcknapsackbudget such that $\WW'$ be the resulting subset of $\VV'$ with (i) $\WW'$ is a \vc of size at most $k'$, (ii) $\sum_{u\in \WW'} w(u) \leq s = k' $, (iii) $\sum_{u\in \WW'} \alpha(u) \geq d = k'$.\\
	\noindent
	This means that the set $\WW'$ is a \vc which gives the maximum profit $k'$ for the bag capacity of $k'$.  Now, since $k'=k$ and $\WW' =\{u_i: v_i \in \WW, \forall i \in[n]\}$ , we can say that  $\WW$ is a \vc of size $k$. Therefore, the \vc instance is an \yes instance.\\
	
	\noindent
	Conversely, let us assume that \vc instance $(\GG,k)$ is an \yes instance.\\ 
	Then there exists a subset $\WW\subseteq \VV$  of size $k$ such that it outputs a \vc. \\	
	\noindent
	Since $\WW' =\{u_i: v_i \in \WW, \forall i \in[n]\}$ and each vertex of $\WW'$ is involved with weight 1 and produces profit amount 1 in the reduced graph $\GG'$, $\WW'$ is a \vc of max bag size and total profit $k$. Also we have, $k=k'$.
	Therefore, the \vcknapsackbudget instance is an \yes instance.\\
\end{proof}


%\subsection{Algorithmic Results}
%\subsubsection{Algorithm}\label{sec:algo_dp_vckp_budget_trees}


    
\begin{comment}
\begin{theorem}\label{thm:vckp_budget_trees-algo}
	There is an algorithm of \vcknapsackbudget with complexity $\OO(n^2\cdot min\{s^2, (\alpha(\VV))^2\})$.
\end{theorem}

\begin{proof}


We denote an arbitrary instance of \vcknapsackbudget by $(\GG,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d,k)$. In this dynamic programming algorithm, we compute a set of all undominated weight-profit pairs of \vc of size $k$ for a graph $\GG$ that also satisfies the knapsack constraints with bag size $s$. Let $\GG=\TT$. We consider $u$ as the root of the tree $\TT$, and $d_u$ is the maximum degree of $u$. We Compute  $D[u,d_u, l]$ and $D[\bar{u},d_u, l]$ from the all the $d_u$ number of children $v_1, v_2,\ldots,v_{d_u}$ recursively, where $D[u,d_u, l]$ is the set of undominated weight-profit pairs of Vertex Covers including $u$ and $D[\bar{u},d_u, l]$ is excluding $u$ also $0 \leq l \leq k$. We Formally define $D[u,d_u, l]=\{(w_c,\alpha_c):\exists$ some $\vc$ $\CC$ with $w(\CC)=w_c<w(\CC')$ and/or $\alpha(\CC)=\alpha_c>\alpha(\CC')$, where $\CC'$ is another \vc such that $|\CC|=|\CC'|=l$ and $u$ is included in both $\CC$ and $ \CC' \}$. $D[\bar{u},d_u, l]$ also carries the same definition but without including $u$. We consider $d_{v_1},d_{v_2},\ldots,d_{v_{d_u}}$ are the maximum degree the next-level children $v_1, v_2,\ldots,v_{d_u}$ of $u$ respectively (See \cref{fig:t1}). After computing $D[u, d_u, l]$ and $D[\bar{u}, d_u, l]$, we remove dominated and duplicated weight-profit pairs from $D[u, d_u, l] \cup D[\bar{u}, d_u, l]$ and  output \YES if a weight-profit pair $(w_c,\alpha_c)$ of \vc $\CC$ exists  in $D[u, d_u, l] \cup D[\bar{u}, d_u, l]$ such that $w_c \leq s$, $\alpha_c \geq d$ and $|\CC|=l$. $D[u, i, l]$ is nothing but an entry of a 2-dimensional DP table with index $i$ and $l$, where we vary $i$ from $0$ to $d_u$ and $l$ from $0$ to $k$.\\

\noindent
\textbf{Initialization:} If $u$ is a leaf node,  maximum degree $(d_u)$ is $0$. We initialize $D[u, 0, l]$ of the DP table of $u$ as $D[u, 0, 0]=\{(0,0)\}$; $D[u, 0, 1]= \{(w(u),\alpha(u))\}$; $D[u, 0, l]= \emptyset$ if $l=2$ to $k$ and $D[\bar{u}, 0, l]$ as $D[\bar{u},0,l]= \emptyset$ for $l=0$ to $k$. For each leaf node, $u \in \VV$, the DP tables containing $u$ and without containing $u$ are 1-D arrays.\\
If  $u$ is a non-leaf node, we set the base conditions for first row, first column and second column of the DP tables $D[u, i, l]$ (containing $u$)  and $D[\bar{u}, i, l]$ (without containing $u$) as follows, where $0\leq i\leq d_u$ and $0\leq l\leq k$. 

	\begin{align*}
	D[u,i, l] &= \begin{cases}
		\left. \begin{aligned}\{(0,0)\} \text{ , } \qquad \qquad \qquad & i=0, l=0 \\
		\{(w(u),\alpha(u))\} \text{ , } \qquad \qquad \qquad & i=0, l=1 \\
		 \emptyset \text{ , } \qquad \qquad \qquad & i=0, 2 \leq l \leq k\\\end{aligned}\right\}\\
		 \left.\begin{aligned}
		 \emptyset \text{ , }\qquad \qquad \qquad \qquad \qquad \qquad  & 1 \leq i \leq d_u , l=0
		\end{aligned}\right\}\\
		\left.\begin{aligned}\begin{cases}
			D[u,i-1, 1] & \text{if } d_{v_i}=0\\
			\emptyset & \text{otherwise}
		\end{cases} \text{ , } \quad & 1 \leq i \leq d_u, l=1 \end{aligned}\right\} \\
	\end{cases}\\
\end{align*}
	\begin{align*}
	D[\bar{u},i, l] &= \begin{cases}
		\left. \begin{aligned}\emptyset \text{ , } \qquad \qquad \qquad \qquad \qquad \qquad & i=0, 0 \leq l \leq k \\
		\end{aligned}\right\}\\
		\left. \begin{aligned}\emptyset \text{ , } \qquad \qquad \qquad \qquad \qquad \qquad & 1 \leq i \leq d_u , l=0\\\end{aligned}\right\}\\
		\left.\begin{aligned}\begin{cases}
			D[v_i, d_{v_i}, 1] & \text{if } i=1\\
			\emptyset & \text{otherwise}
		\end{cases} \text{ , } \quad & 1 \leq i \leq d_u, l=1\end{aligned}\right\}\\
	\end{cases}\\
\end{align*}
The first row $(i=0)$ initialization for both $D[u, i, l]$ and $D[\bar{u}, i, l]$ is the same as the initialization of leaf nodes. For $D[u,i, l]$ and $1 \leq i \leq d_u$, first column: $D[u,i, 0]= \emptyset$; second column: $D[u,i, 1]=D[u,i-1, 1]$, if $d_{v_i}=0$; otherwise $D[u,i, 1]= \emptyset$. Now, for $D[\bar{u},i, l]$ and $1 \leq i \leq d_u$, first column: $D[\bar{u},i, 0]= \emptyset$;  second column: $D[\bar{u},1, 1]=D[v_i,d_{v_i},1]$, if i=1; $D[\bar{u},i, 1]=\emptyset$, otherwise.\\

\noindent
\textbf{Updating DP table:} The DP tables D[$v_i, d_{v_i}, k$] and D[$\bar{v_i}, d_{v_i}, k$] for each child $v_i$ of $u$ are computed recursively for each child $v_i$ of $u$. Now, we update $D[u, i,l]$ for all the values of $i \in [1, d_u]$ and $l \in [2, k]$ based on the already-computed table entry of the children of $u$ and the entry of $(i-1)^th$ row of the table of $u$. We first initialize $D[u, i, l] =\emptyset$. Then update $D[u, i, l]$ to $D[u,i,l]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$ for each non-null pair $(w_1, \alpha_1) \in D[u, i-1, l_1] $ and for each non-null pair $(w_2, \alpha_2) \in D[v_i, d_{v_i}, l-l_1]\cup D[\bar{v_i}, d_{v_i}, l-l_1] $, where $l_1= 0$ to $l$. We are taking $l_1$ in this way because we are trying to find and store a \vc of size $l$ in $D[u, i, l]$. So, we choose weight-profit pairs of \vc from $(i-1)^th$ row-entry of the table of $u$, say, $(w_1, \alpha_1)$ with the table entry of the children of $u$, say, $(w_2, \alpha_2)$ for summing up in such a way that the resulting size of the \vc does not exceed the size $l$, where $0 \leq l \leq k$.\\ The similar thing we do for $D[\bar{u},i,l]$ for all the values of $i \in [1,d_u]$ and $l \in [2, k]$.  After initializing $D[\bar{u},i,l]=\emptyset$, we update $D[\bar{u}, i, l]$ to $D[\bar{u}, i, l]\cup\{(w_3+w_4,\alpha_3+\alpha_4)\}$ for each non-null pair $(w_3, \alpha_3) \in D[\bar{u}, i-1, l-l_2] $ and each non-null pair $(w_4, \alpha_4) \in D[v_i,d_{v_i}, l_2 ] $, where $l_2=1$ to $l$.\\

\noindent
\textbf{Correctness:} We get the final set $\FF$ of undominated weight-profit pair of Vertex Covers, after removal of all dominated and duplicated pairs from $D[u, d_u, k] \cup D[\bar{u}, d_u,k]$ such that $w_c \leq s$, $\alpha_c \geq d$ and size of each \vc is $k$.  Now we will prove that an arbitrary pair $(w_c,\alpha_c) \in \FF$, is a \vc $\CC$ such that $w(\CC)=w_c$, $\alpha(\CC)=\alpha_c$ and $|\CC|=l$, where $l \in [0, k]$. Let us consider $\exists$ an arbitrary pair $(w_c,\alpha_c) \in \FF$. In the above algorithm, if $v$ is leaf node, we choose $ (w_c,\alpha_c)$ either from $D[v, 0, 0]=\{(0,0)\}$ or from $D[v, 0, 1]= \{(w(v)),\alpha(v))\}$ or from $D[v, 0, l]= \emptyset$ if $l=2$ to $k$ or from $D[\bar{v},0,l]= \emptyset$ for $l=0$ to $k$. So, every set satisfies the above hypothesis trivially. Let us suppose $v_j$ is a non-leaf node, and it is the $j^{th}$ child of the root node $u$ and for all $j= 1$ to $d_u$, $D[v_j, d_{v_j}, l] \cup D[\bar{v_j},d_{v_j}, l]$ gives the sets of undominated weight-profit pair of Vertex Covers at (root-level -1), for $l=0$ to $k$. Now, for the root node $u$, we compute $D[u, d_u, l]$ and  $D[\bar{u}, d_u, l]$. From the above algorithm, each pair $(w_2, \alpha_2) \in D[v_j,d_{v_j}, l]\cup D[\bar{v_j},d_{v_j}, l]$ is \vc of size $l$, where $l \in [0, k]$. Moreover, each pair $(w_1, \alpha_1) \in D[u,j-1, l]$ is the entry of $(j-1)^th$ row of the table of $u$ and have calculated from $0^{th}$ to $(j-1)^{th}$ subtree of $u$ ($v_1$ to $v_{j-1}$ including $u$), so $(w_1, \alpha_1)$ also be a vertex cover of size $l \in [0, k]$, as for trees there is no overlapping of two subtrees. Since we sum up the pairs $(w_1+w_2,\alpha_1+\alpha_2)$ for \vc, they can be of size $\geq k $. However, we can argue that our given algorithm updates a table entry $D[u, i, l]$ to $D[u, i, l]\cup\{(w_1'+w_2',\alpha_1'+\alpha_2')\}$ for each non-null pair $(w_1', \alpha_1') \in D[u, i-1, l_1] $ and for each non-null pair $(w_2', \alpha_2') \in D[v_i, d_{v_i}, l-l_1]\cup D[\bar{v_i}, d_{v_i}, l-l_1] $, where $l_1= 0$ to $l$ in such a way that for $D[u, i, l]$ we get sets of \vc of size $l$ only. Because, here, we are taking $l_1$ in this way that we can try to find and store a \vc of size $l$ in $D[u, i, l]$. So, we choose weight-profit pairs of \vc from $(i-1)^{th}$ row-entry of the table of $u$, say, $(w_1', \alpha_1')$ with the table entry of the children of $u$, say, $(w_2', \alpha_2')$ for summing up in such a way that the resulting size of the \vc does not exceed the size $l$, where $0 \leq l \leq k$.
The same thing happen when we consider $D[\bar{u}, i, l]$ where, $i \in [0, d_u]$ and $l \in [0, k]$. Thus, we get a \vc $\CC$ with $w(\CC)=w_c$, $\alpha(\CC)=\alpha_c$ and $|\CC|=l$, where $0 \leq l \leq k$ for some arbitrary pair $(w_c, \alpha_c)$. Thus, by considering the hypothesis TRUE in (root -1)$^{th}$ level, we proved by induction that it is also TRUE for the root node. \\

\noindent
\textbf{Complexity:}
For each $n$ vertices we are computing $D[u,d_{u}, l]$ and $D[\bar{u},d_{u}, l]$, where $0 \leq l \leq k$ for all $u \in \VV$. In computation of $D[u,d_{u}, l]$ we store   $D[u,j, l]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$ to $D[u,j]$for each pair $(w_1, \alpha_1) \in D[v_j,d_{v_j}, l]\cup D[\bar{v_j},d_{v_j}, l]$ and each pair $(w_2, \alpha_2) \in D[u,j-1, l]$. So, this part gives the complexity $\OO( min\{s, (\alpha(\VV))\})$ as each table entry can contain at most $min\{s, (\alpha(\VV))\}$ pairs and we are merging two sorted lists and similarly for  $D[\bar{u},d_{u}, l]$. Hence the total complexity is $\OO(n\cdot k \cdot min\{s, (\alpha(\VV))\})$ = $\OO(n^2 \cdot min\{s, (\alpha(\VV))\})$ as $k$ can be at most $n$.
\end{proof}

    
\end{comment}

\begin{comment}


\break
\textbf{COMPUTE} D[$u, d_u, k$]
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		%\State $\textbf{T(u,d_u)}$
		\If{$u$ is a leaf node} \textcolor{blue}{\Comment{ \textit{/* If ~ $u$ is a leaf node */}}}
		\If{$l==0$}
		\State $D[u, 0, 0]\leftarrow \{(0,0)\}$;
		
		\ElsIf{$l==1$}
		\State $D[u, 0, 1]\leftarrow \{(w(u),\alpha(u))\}$;
		\Else
		\For{$l=2$ to $k$}
		\State $D[u, 0, l]\leftarrow \emptyset$;
		\EndFor
		\EndIf
		
		\State \textbf{return DPTable}$[u,0,k]$;
		\Statex
		\Else \textcolor{blue}{\Comment{ \textit{/* If ~ $u$ is a non-leaf node */}}}
		\Statex
		\Statex
		%\State\textcolor{red}{ $Temp\leftarrow\emptyset$;}
		%\State $D[u,0]\leftarrow\{(w(u),\alpha(u))\}$
		
		%\For{ $i=1$ to $k$}
		\For{$i=0$ to $d_u$}
		%\For{$l=0$ to $k$}
		
		\Statex
		\If{$i==0$}  \textcolor{blue}{\Comment{ \textit{/* Base condition for the $1^{st}$ row. */}}}
		\If{$l==0$}
		\State $D[u, 0, 0]\leftarrow \{(0,0)\}$;
		
		\ElsIf{$l==1$}
		\State $D[u, 0, 1]\leftarrow \{(w(u),\alpha(u))\}$;
		\Else
		\For{$l=2$ to $k$}
		\State $D[u, 0, l]\leftarrow \emptyset$;
		\EndFor
		\EndIf
		\Statex
		
		\Else \textcolor{blue}{\Comment{ \textit{/* For the rows other than $1^{st}$ row, i.e., $i \geq 1$ */}}}
		\Statex
		\If{$l==0$} \textcolor{blue}{\Comment{ \textit{/* Base condition for the $1^{st}$ column. */}}}
		\State $D[u, i, 0]\leftarrow \emptyset$;
		\Statex
		\ElsIf{$l==1$} \textcolor{blue}{\Comment{ \textit{/* Base condition for the $2^{nd}$ column. */}}}
		\If{$d_{v_i}==0$}
		\State $D[u, i, 1]\leftarrow D[u, i-1, 1]$;
		\Else %\Comment{this is a comment}
		\State $D[u, i, 1]\leftarrow \emptyset$;
		\EndIf
		\EndIf
		
		\Statex
		\State \textbf{COMPUTE} D[$v_i, d_{v_i}, k$]; \textcolor{blue}{\Comment{ \textit{/* Computing dp table for $i^{th}$ vertex of ~$u$ */}}}
		\State \textbf{COMPUTE} D[$\bar{v_i}, d_{v_i}, k$];
		
		\Statex
		
		\For{$l=2$ to $k$}
		\State $D[u,i,l]\leftarrow\emptyset$; \textcolor{blue}{\Comment{ \textit{/* Initialization for ~$i\geq 1, l \geq 2$ */}}}
		
		\For{$l_1=0$ to $l$} 
		\For{each non-null pair $(w_1, \alpha_1) \in D[u, i-1, l_1] $}
		\For{each non-null pair $(w_2, \alpha_2) \in D[v_i,d_{v_i}, l-l_1]\cup D[\bar{v_i},d_{v_i},l-l_1] $}
		\State$D[u,i,l]\leftarrow D[u,i,l]\cup\{(w_1+w_2,\alpha_1+\alpha_2)\}$;
		
		
		\EndFor
		\EndFor
		\EndFor
		%\State \textcolor{red}{$D[u,j]\leftarrow Temp$;}
		%\State \textcolor{red}{$Temp\leftarrow\emptyset$;}
		\State Remove dominated and duplicate pairs from $D[u,i,l]$;\textcolor{blue}{\Comment{ \textit{/* Generated the set of pairs for ~$i\geq 1, l \geq 2$ */}}}
		\EndFor
		\Statex
		\EndIf
		\Statex
		\EndFor
		%\EndFor
		\Statex
		\State \textbf{return DPTable}$[u,d_u,k]$;
		\Statex
		\Statex
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}


%\end{Algorithms}
The function \textbf{COMPUTE} D[$u, d_u, k$] returns all undominated weight-profit pairs, which are individually a solution of a \vc that must include $u$ of size $k$. Lines 1 to 11 execute if $u$ is a leaf node; otherwise, lines 12 to 49 execute. In lines 34, 35 \textbf{COMPUTE} D[] function executes recursively to find undominated \vc pairs for each of the child of $u$.

\textbf{COMPUTE} D[$\bar{u}, d_u, k$]
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		%\State $\textbf{T(u,d_u)}$
		\If{$u$ is a leaf node} \textcolor{blue}{\Comment{ \textit{/* If ~ $u$ is a leaf node */}}}
		\For{$l=0$ to $k$}
		\State $D[\bar{u},0,l]\leftarrow \emptyset$;
		\EndFor
		\State \textbf{return DPTable}$[\bar{u},0,k]$;
		
		
		\Statex
		\Else \textcolor{blue}{\Comment{ \textit{/* If ~ $u$ is a non-leaf node */}}}
		\Statex
		
		%\State $D[\bar{u},0]\leftarrow\{(0,0)\}$
		\For{$i=0$ to $d_u$}
		
		\Statex
		%\State $D[\bar{u},i]\leftarrow\emptyset$;
		\If{$i==0$} \textcolor{blue}{\Comment{ \textit{/* Base condition for the $1^{st}$ row. */}}}
		\For{$l=0$ to $k$}
		\State $D[\bar{u},0,l]\leftarrow\emptyset$;
		\EndFor
		
		\Statex	
		\Else \textcolor{blue}{\Comment{ \textit{/* For the rows other than $1^{st}$ row. */}}}
		\If{$l==0$} \textcolor{blue}{\Comment{ \textit{/* Base condition for the $1^{st}$ column. */}}}
		\State $D[\bar{u}, i, 0]\leftarrow \emptyset$;
		
		\ElsIf{$l==1$} \textcolor{blue}{\Comment{ \textit{/* Base condition for the $2^{nd}$ column. */}}}
		\If{$i==1$}
		\State $D[\bar{u}, 1, 1]\leftarrow D[v_i, d_{v_i}, 1]$;
		\Else
		\State $D[\bar{u}, i, 1]\leftarrow \emptyset$;
		\EndIf
		
		\EndIf
		
		\Statex
		\For{$l=2$ to $k$} 
		\State $D[\bar{u},i,l]\leftarrow\emptyset$; \textcolor{blue}{\Comment{ \textit{/* Initialization for ~$i\geq 1, l \geq 2$ */}}}
		
		\For{$l_2=1$ to $l$}
		\For{each non-null pair $(w_3, \alpha_3) \in D[\bar{u}, i-1, l-l_2] $}
		\For{each non-null pair $(w_4, \alpha_4) \in D[v_i,d_{v_i}, l_2 ] $}
		
		\State$D[\bar{u}, i, l]\leftarrow D[\bar{u}, i, l]\cup\{(w_3+w_4,\alpha_3+\alpha_4)\}$;
		\EndFor
		\EndFor
		\EndFor
		
		\State Remove dominated and duplicate pairs from $D[\bar{u},i,l]$; \textcolor{blue}{\Comment{ \textit{/* Generated the set of pairs for ~$i\geq 1, l \geq 2$ */}}}
		\EndFor
		
		\EndIf
		\EndFor
		
		\State \textbf{return DPTable}$[\bar{u},d_u,k]$; 
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}
%\end{Algorithms}
%\parskip 2em
Similarly, \textbf{COMPUTE} D[$\bar{u}, d_u$] returns the solution pairs of \vc that must not include $u$.\\

\textbf{VCKnapsackWithBudget}($\TT, s, u, d_u, k$)
\begin{breakablealgorithm}\label{}
	%\caption{$\textbf{\pa}$ ($T$, $(r_u)_{u\in\VV}$, $(\alpha_u)_{u\in\VV}$, $x$, $r_a$, $n$)}
	\hspace*{\algorithmicindent}
	\begin{algorithmic}[1]	
		
		\State \textbf{COMPUTE} D[$u, d_u, k$];
		\State \textbf{COMPUTE} D[$\bar{u}, d_u, k$];
		\State Remove dominated and duplicate weight-profit pairs from $D[u, d_u, k] \cup D[\bar{u}, d_u, k]$ such that each weight $\leq s$;
		\For{$l=0$ to $ k$}
		\State \textbf{VCKB $[\TT, u, l]$}= $D[u, d_u, l] \cup D[\bar{u}, d_u, l]$;
		\EndFor
		\State \textbf{return} \textbf{VCKB $[\TT, u, k]$};
	\end{algorithmic}
\end{breakablealgorithm}
The function \textbf{VCKnapsackWithBudget} calls the two recursive functions in lines 1 and 2. After getting the two undominated solution pair sets again, we remove the dominating pairs from $D[u, d_u] \cup D[\bar{u}, d_u]$ and we check the condition of the knapsack size $s$ so that the knapsack can contain them individually in line 3. Finally, we get our desired solution, an 1-D array in line 7.
\end{comment}


%\break
\subsection{\minimalvcknapsack}\label{sec:res3c}
%\subsection{Hardness Results}
We show that \minimalvcknapsack is strongly \NPC by reducing it from \maxminimalvc which is a \NPC problem. 

\begin{theorem}\label{thm:minimalvckp-gen-npc}
	\minimalvcknapsack is strongly \NPC for general graph.
\end{theorem}

\begin{proof}
	Clearly, \minimalvcknapsack $\in$ \NP. Since, the decision version of \maxminimalvc is \NPC,  we reduce \maxminimalvc to \minimalvcknapsack to prove NP-completeness. Let $(\GG(\VV=\{v_i: i\in[n]\},\EE),k)$ be an arbitrary instance of \maxminimalvc of size $k$. We construct the following instance $(\GG^\pr(\VV^\pr=\{u_i: i\in[n]\},\EE^\pr),(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d)$ of \minimalvcknapsack.
	\begin{align*}
		&\VV^\pr = \{u_i : v_i\in \VV, \forall i\in[n]\}\\
		&\EE^\pr = \{\{u_i,u_j\}: \{v_i, v_j\} \in\EE, i\neq j, \forall i, j\in[n]\}\\
		&w(u_i) = 1, w(u_j)=0 \quad \text{for~some~} i,j \in [1,n] \\
		&\alpha(u_i)=1 \quad \forall i \in [1,n] \\
		&s = d =k\\
	\end{align*}
	The reduction of \maxminimalvc to \minimalvcknapsack works in polynomial time. The \minimalvcknapsack problem has a solution iff \maxminimalvc has a solution.\\
	\noindent
	Let $(\GG^\pr(\VV^\pr,\EE^\pr),(w(u))_{u\in\VV^\pr},(\alpha(u))_{u\in\VV^\pr},s,d)$ of \minimalvcknapsack such that $\WW$ be the resulting subset of $\VV'$ with (i) $\WW$ is a minimal \vc, (ii) $\sum_{u\in \WW} w(u) \leq s = k$, (iii) $\sum_{u\in \WW} \alpha(u) \geq d = k$.\\
	From the above condition (i), as $\WW$ is minimal \vc we can not remove any vertex from $\WW$ which gives another \vc. Now, since we rewrite the second and third conditions as $|\WW| \leq k$ and $|\WW| \geq k$. So, $|\WW|$ must be $k$. Now, let $\II=\{v_i:u_i \in \WW,\forall i\in[n]\}$. Since $\WW$ is the Minimal \vc of size $k$, then $\II(\subseteq \VV)$ must be \maxminimalvc set of size at least $k$.Therefore, the \maxminimalvc instance is an \yes instance.\\
	
	\noindent
	Conversely, let us assume that \maxminimalvc instance $(\GG,k)$ is an \yes instance.\\ 
	Then there exists a subset $\II\subseteq \VV$  of size $ \geq k$ such that it outputs an \maxminimalvc. Let $\WW=\{u_i:v_i \in \II,\forall i\in[n]\}$. Since $\II$ is an \maxminimalvc of size $ \geq k$, then $\WW$ must be a Minimal \vc of size $k$. So, $\sum_{u\in \WW} w(u) \leq k =s$ and $\sum_{u\in \WW} \alpha(u) \geq k = d$. Now, we want to prove that $\WW$ is a minimal \vc.\\
	\noindent
	Therefore, the \minimalvcknapsack instance is an \yes instance.\\
\end{proof}

\begin{theorem}\label{minimalvck-trees-npc}
\minimalvcknapsack is \NPC for trees.
\end{theorem}

\begin{proof}
Clearly, \minimalvcknapsack for tree $\in$ NP.
\begin{comment}, i.e. given \UU $\subseteq$ \VV, it can be verified in polynomial time if:
\begin{enumerate}
		\item \UU is a minimal \vc,
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
\end{enumerate}
\end{comment}
We reduce \minimalvcknapsack from \kp to prove hardness. Given, an arbitrary instance $(\XX,(\theta_i)_{i\in\XX}, (p_i)_{i\in\XX}, b,q)$ of \kp,  we create an instance of \minimalvcknapsack for trees by forming a complete binary tree \TT = (\VV, \EE) that has $n$ nodes in its penultimate level and denote an instance as $(\TT,(w(u))_{u\in\TT},(\alpha(u))_{u\in\TT},s,d)$. The construction steps is as follows:

\begin{enumerate}
    \item We construct a complete binary tree \TT such that the penultimate level of this tree has $n$ nodes representing the $n$ items.
    \item Without loss of generality we assume, that $n=|\XX|=2^k$ because suppose there exists $n$ such that $2^{k-1} < n < 2^{k} $, add  $2^{k} - n$ items to \XX each with size = 0 and profit = 0, where $k \ge 0$. 
    \item Let $\VV^\pr \subseteq \TT[\VV]$ denote the vertices belonging to the penultimate level of the tree \TT.
    \item Set $w(u_i)_{u_i \in \VV^\pr} = \theta_i, \alpha(u_i)_{u_i \in \VV^\pr} = p_i, 
			w(u_i)_{u_i \in \VV - \VV^\pr}=0, \alpha(u_i)_{u_i \in \VV - \VV^\pr}=0 \\
			s=b, d=q$
\end{enumerate}

\begin{comment}
\begin{enumerate}
    \item Construct \TT(\VV, \EE) as:
    \begin{align*}
			&\VV =  \{u_{ik}: \forall x_i \in \XX \} \cup \\
   &\hspace{0.9cm}\{u_{i(k-j)}: (u_{(2i-1)(k-j+1)}, u_{(2i)(k-j+1)}) \in \TT, i \in [\log (k-j+1)], j \in [k-1]\} \cup   \\
   &\hspace{0.9cm}\{u_{i(k+1)}, u_{2i(k+1)}: \forall u_{ik}\} \\
			&\EE = \{\{u_{ij},u_{(2i-1)(j+1)}\}:  i \in [2^{j-1}], j \in [k] \}
			\cup \\
   &\hspace{0.9cm}\{\{u_{ij},u_{(2i)(j+1)}\}:  i \in [2^{j-1}], j \in [k] \} \\
                &\VV^\pr =  \{ u_{ik}: \forall x_i, \in \XX \} \\
			&w(u_i)_{u_i \in \VV^\pr} = \theta_i, \alpha(u_i)_{u_i \in \VV^\pr} = p_i, 
			w(u_i)_{u_i \in \VV - \VV^\pr}=0, \alpha(u_i)_{u_i \in \VV - \VV^\pr}=0 \\
			&s=b, d=q
\end{align*}
\end{enumerate}
\end{comment}
This construction takes polynomial time.
\par We now show that \kp $\le_p$ \minimalvcknapsack.

The \minimalvcknapsack problem has a solution if and only if \kp has a solution.

\minimalvcknapsack ~ \ding{222} \kp \\
Let $(\TT,(w(u))_{u\in\VV},(\alpha(u))_{u\in\VV},s,d)$ be an instance of \minimalvcknapsack such that $\WW$ be the resulting subset of $\VV$ with
	\begin{enumerate}
		\item $\WW$ is a minimal \vc,
		\item $\sum_{u\in \WW} w(u) = b$,
		\item $\sum_{u\in \WW} \alpha(u) = d$
	\end{enumerate}
	This means that the set $\WW$ is a minimal \vc, which gives the maximum profit $d$ for the bag capacity of size $b$. In other words, $\WW \cap \VV^\pr = \WW^\pr \ne \phi$ i.e. \WW must contain at least a subset of $\VV^\pr$ in order to attain the required profit $d$ because \WW - \VV' has vertices whose weight = 0, and profit = 0. As per our construction, \VV' contains the vertices denoting the $n$ items of \XX in \kp.
	\noindent
	Therefore, the \kp instance is an \yes instance.\\

 
 \kp ~ \ding{222} \minimalvcknapsack \\
Let $(\XX,(\theta_i)_{i\in\XX}, (p_i)_{i\in\XX}, b,q)$ be an instance of \kp such that $\II$ be the resulting subset of $\XX$ with
	\begin{enumerate}
		\item $\sum_{i\in \II} \theta_i \leq b$,
		\item $\sum_{i\in \II} p_i \geq q$
	\end{enumerate}
	The minimal vertex cover knapsack must pick vertices from $\VV^\pr$ otherwise it cannot meet the desired value $d$ as all vertices of $\VV - \VV^\pr$ have weight and value equal to 0.
 

 We obtain a minimal \vc for \TT by recursively constructing the solution set, \WW as:
\begin{enumerate}
     \item if $u \in \TT[\II]$, include $u$ in \WW and delete $\NN[u]$ from \TT
     \item if $u \notin \TT[\II]$, include $\NN(u$ in \WW delete $\NN[u]$ from \TT 
     \item solve for minimal vertex cover on the induced sub-graph where weight and profit associated with each vertex is 0.   
 \end{enumerate}     

 
\noindent
	Therefore, the \minimalvcknapsack for tree is an \yes instance.\\

\end{proof}
%\break
\subsection{\minimumvcknapsack}\label{sec:res3d}

\begin{observation}\label{obs:minvckp-not-poly}
	This problem is not known to be in \NP, even the decision version of this problem for the general graph.
\end{observation}

\section{Results: Polynomial Time Approximation Algorithms}
\label{approximation}
In this section, we define optimization versions of the \vcknapsack problem. We consider the following two versions:

\begin{definition}[\vcktp]\label{vcktp}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, and target value $d$, compute a subset $\UU\subseteq\VV$ of vertices that minimizes the total weight $w(\UU)=\sum_{u\in\UU} w(u)$ such that:
	\begin{enumerate}
		\item \UU is a vertex cover.
		%\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
\end{definition}


\begin{definition}[\vckmb]\label{vckmb}
	Given an undirected graph $\GG=(\VV,\EE)$, weight of vertices $(w(u))_{u\in\VV}$, value of vertices $(\alpha(u))_{u\in\VV}$, and size $s$ of knapsack, compute a subset $\UU\subseteq\VV$ of vertices that maximizes the total value $\alpha(\UU) = \sum_{u\in\UU} \alpha(u) $such that:
	\begin{enumerate}
		\item \UU is a vertex cover.
		\item $w(\UU)=\sum_{u\in\UU} w(u) \le s$,
		%\item $\alpha(\UU)=\sum_{u\in\UU} \alpha(u) \ge d$
	\end{enumerate}
\end{definition}

We formulate \vcktp problem as the following integer linear programming, in which the primal variable $x_i$ indicates whether vertex $v_i \in \VV$ is chosen to be in the solution or not:

minimize $\sum_{u \in \VV} w(u)x_u$ 
\begin{align*}
    \text{Subject to:}\\
       &x_u + x_v \geq 1,\forall (u,v) \in \EE \\
        &\sum_{u\in \VV} \alpha(u)x_u \geq d \\
    &x_u \in \{0,1\}, \forall u \in \VV
\end{align*}


We replace the constraints $x_u \in \{0,1\}$, with $x_u \geq 0$, $\forall u \in \VV$ to obtain linear programming relaxation of the integer linear program.
\begin{observation}
    The relaxed linear programming of the above integer linear programming has an unbounded integrality gap.  Consider an edgeless graph \GG(\VV, \EE) such that $\EE = \emptyset$. Let $\VV = \{v_1, v_2\}$, $w(v_1) = 0$, $w(v_2) = 1$, $\alpha(v_1) = d-1$ and $\alpha(v_2) = d$. The optimal solution to integer linear programming sets $x_{v_1} = 0, x_{v_2} = 1$, for a total weight of 1. However, the solution to the relaxed linear programming sets $x_{v_1} = 1, x_{v_2} = 1/d$ and has total weight of 1/d. Thus, in this case the integrality gap is at least $\frac{1}{1/d} = d$. 
\end{observation}
We also consider a generalized version of \vc problem i.e. \setc problem. 

\begin{definition}[\setc]\label{setcover}
	Given a universe \UU of $n$ elements and some subsets $\SS_1, \SS_2, \dots, \SS_m$ where each $\SS_i \subseteq \UU$, and a non negative weight $w(i) \ge 0$  for each subset $\SS_i$, $\forall i \in [m]$. The goal is to find $\II \subseteq \{1, 2, \dots, m\}$ that minimizes $\sum_{i\in\II} w(i)$ subject to $\bigcup_{i \in \II} \SS_i = \UU$ .
\end{definition}

Vertex cover is a special case of set cover. Interestingly, if each set $\SS_i$, $\forall i \in [m]$, is assigned with a non-negative value in addition to weight, and we look for a solution to the \setc that not only minimizes the weight but also maximizes the value, then we call this problem as \setck. Now it is easy to see that, \setck problem is also \NPC and hence we cannot hope to have a deterministic polynomial time algorithm unless $P \neq \NP$. The optimization versions of the \setck problem are \setckp and \setcks. In \setckp, the desired solution must be a solution to the \setc problem and must meet the desired value, say $d$ with minimum weight. On the other hand, the solution to the \setcks problem, must maximize the value while not exceeding the given weight, say $s$. We formally define the problems below.

\begin{definition}[\setckp]\label{setcoverkp}
	Given a universe \UU of $n$ elements and a family of subsets $\FF = \{1, 2, \dots, m\}$ where each $\SS_i \subseteq \UU$, $\forall i \in [m]$ and a non negative weight $w(i) \ge 0$ and value $\alpha(i) \ge 0$ for each subset $\SS_i$, $\forall i \in [m]$. The goal is to find $\II \subseteq \{1, 2, \dots, m\}$ that minimizes $\sum_{i\in\II} w(i)$ subject to $\bigcup_{i \in \II} \SS_i = \UU$ such that the total value is at least $d$.
\end{definition}

\begin{definition}[\setcks]\label{setcoverks}
	Given a universe \UU of $n$ elements and a family of subsets $\FF = \{1, 2, \dots, m\}$ where each $\SS_i \subseteq \UU$, $\forall i \in [m]$, and a non negataive weight $w(i) \ge 0$ and value $\alpha(i) \ge 0$ for each subset $\SS_i$, $\forall i \in [m]$. The goal is to find $\II \subseteq \{1, 2, \dots, m\}$ that maximizes $\sum_{i\in\II} \alpha(i)$ subject to $\bigcup_{i \in \II} \SS_i = \UU$ such that the total weight is at most $s$.
\end{definition}

Till now we have considered the \vcknapsack problem for planar graphs. We now generalise the problem for hyper-graphs using \hs. The \hs problem is one of the fundamental combinatorial optimization problems: given a set of points \PP and a set of geometric objects \DD in the plane, the goal is to compute a small-sized subset of \PP that hits all objects in \DD \cite{bus2018practical}. This problem suitably capture the vertex cover problem on hyper-graphs \cite{durocher2015duality}. 


\begin{definition}[\hs]\label{hs}
	Given a universe \UU of $n$ elements and a family of subsets $\FF = \SS_1, \SS_2, \dots, \SS_m$ where each $\SS_i \subseteq \UU$ $\forall i \in [m]$, $|\SS_i| \leq $ d, and a non negative weight $w(j) \ge 0$  for each element $j$, $\forall j \in [n]$. The goal is to find $\JJ \subseteq \{1, 2, \dots, n\}$ that minimizes $\sum_{j\in\JJ} w(j)$ such that each subset $\SS_i$ is hit by some element in \JJ.
\end{definition}

It is easy to see that \setc is dual to \hs, meaning that it is exactly the same problem, i.e we are looking for a set cover in the dual set system.
There is a $\rho$ factor approximation algorithm for \hs if and only if there is a $\rho$ factor approximation algorithm for \setc \cite{Skiena2008}. Similar to the \setck, we can formulate \hs KNAPSACK problem. In the \hs problem we assign values and weights to the elements of the Universe. 


\begin{definition}[\hstp]\label{hstp}
	Given a universe \UU of $n$ elements and a family of subsets $\FF = \SS_1, \SS_2, \dots, \SS_m$ where each $\SS_i \subseteq \UU$ $\forall i \in [m]$, $|\SS_i| \leq $ d, and a non negative weight $w(j) \ge 0$ and a non negative value $\alpha(j)$, $\forall j \in [n]$. The goal is to find $\JJ \subseteq \{1, 2, \dots, n\}$ that minimizes $\sum_{j\in\JJ} w(j)$ such that each subset $\SS_i$ is hit by some element in \JJ and the total value is at least $d$.
\end{definition}


\begin{definition}[\hsmb]\label{hsmb}
	Given a universe \UU of $n$ elements and a family of subsets $\FF = \SS_1, \SS_2, \dots, \SS_m$ where each $\SS_i \subseteq \UU$ $\forall i \in [m]$, $|\SS_i| \leq $ d, and a non negative weight $w(j) \ge 0$ and a non negative value $\alpha(j)$, $\forall j \in [n]$. The goal is to find $\JJ \subseteq \{1, 2, \dots, n\}$ that maximizes $\sum_{j\in\JJ} \alpha(j)$ such that each subset $\SS_i$ is hit by some element in \JJ and the total weight is at most $s$.
\end{definition}


We now focus on the \setc problem due to the ease of exposition. We formulate \setckp problem as the following integer linear programming, in which the primal variable $x_i$ indicates whether set $\SS_i$ is chosen to be in the solution or not:

minimize $\sum_{i\in [m]} w(i)x_i$ 
\begin{align*}
    \text{Subject to:}\\
       &\sum_{i:e_j \in \SS_i}x_i \geq 1,\forall e_j \in \UU \\
        &\sum_{i\in [m]} \alpha(i)x_i \geq d \\
    &x_i \in \{0,1\}, \forall i \in [m]
\end{align*}

The above formulation has a bad integrality gap. We think of an alternative formulation where for each subset $\AA \subseteq \FF$ of sets such that $\alpha(A) = \sum_{i \in A} \alpha(i) < d$. We define the residual value $d_\AA = d - \alpha(\AA)$. Given the set \AA, we simplify the problem on the sets $\FF-\AA$, where the target value is is now $d_\AA$. We also reduce the value of the each set $\SS_i \in \FF-\AA$ to be the minimum of its own value and $d_\AA$ i.e let $\alpha^\AA(i)$ = min($\alpha(i)$, $d_\AA$). We can now give the following Integer linear programming formulation of the problem:

minimize $\sum_{i\in [m]} w(i)x_i$ 
\begin{align*}
    \text{Subject to:}\\
       &\sum_{i:e_j \in \SS_i}x_i \geq 1, \forall e_j \in \UU \\
        &\sum_{i\in \FF-\AA} \alpha^\AA(i)x_i \geq d_\AA, \forall \AA \subseteq \FF \\
    &x_i \in \{0,1\}, \forall i \in [m]
\end{align*}
We replace the constraints $x_i \in \{0,1\}$, with $x_i \geq 0$ to obtain linear programming relaxation of the integer linear program. The dual of the linear programming relaxation is :

maximize $\sum_{\AA: \AA \subseteq \FF} d_\AA y_\AA$ + $\sum_{j\in[n]}y_j$
\begin{align*}
    \text{Subject to:}\\
       &\sum_{j:e_j \in \SS_i}y_j \leq w(i), \forall \SS_i \in \FF \\
        &\sum_{\AA\subseteq\FF: i \not\in \AA} \alpha^\AA(i)y_\AA \leq w(i), \forall i \in \FF \\
    &y_\AA \geq 0, \forall \AA \subset \FF
\end{align*}

We can now give a primal dual algorithm in Algorithm \ref{pdsc} for the \setckp problem by modifying the algorithm given in \cite{williamson2011design} using the primal dual formulations given above. 
\begin{algorithm}
\caption{Primal Dual algorithm for the \setckp problem}
\begin{algorithmic}[1]
\State $y \gets 0$
\State $\AA \gets \emptyset$
\While{$\alpha(\AA) < d$}
    \State Increase $ y_\AA$ until for some $i \in \FF - \AA, \sum_{\BB\subseteq\FF: i \not\in \BB} \alpha^\BB(i)y_\BB \leq w(i)$
    \State $\AA \gets \AA \cup \{i\}$
\EndWhile
\State $\XX \gets \AA$
\State $\AA^\pr \gets \AA$
\While{$\exists e_j \not \in \bigcup_{i \in \AA^\pr} \SS_i$}
    \State Increase $y_j$ until there is some $l$ with $e_j \in \SS_l$ such that $\sum_{j:e_j \in \SS_l}y_j \leq w(l) $
    \State $\AA^\pr \gets \AA \cup \{l\}$
\EndWhile
\State \textbf{return} $\AA^\pr$
\end{algorithmic}
\label{pdsc}
\end{algorithm}

\begin{theorem}\label{thm:approxf}
	Algorithm \ref{pdsc} is a $f$-approximation algorithm for the \setckp problem, where $f$ is the frequency of the most frequent element.
\end{theorem}

\begin{proof}
Let $\AA^\pr$ be the output set of our algorithm that contains the indices of the sets that are picked up. Suppose our algorithm returns $ALG$ 

\begin{align}
    ALG &= \sum_{i\in \AA^\pr} w(i)x_i \\
        &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \mathcal{A}^\prime - \mathcal{X}} w(i)x_i 
\end{align}


Let \opt be the optimal solution to the \setckp problem $l$ be the final set selected by the algorithm after termination of the first while loop, and let \XX be the sets returned at the end of the first while loop. Since the while condition terminates when $\alpha(\AA) \geq d$, we know that $\alpha(\XX) \geq d$; since set $l$ was added to $\XX$, it must be the case that before $l$ was added, the total value of the set of items was less than $d$, so that $\alpha(\XX - \{l\}) < d$. 
Following the standard primal-dual analysis, we know that

\begin{equation}
   \sum_{i \in \XX} w(i) = \sum_{i \in \XX} \sum_{\AA \subseteq \FF: i \notin \AA} \alpha^\AA(i) y_\AA. 
\end{equation}


Reversing the double sum, we have that

\begin{equation}
\sum_{i \in \XX} \sum_{\AA \subseteq \FF: i \notin \AA} \alpha^\AA(i) y_\AA = \sum_{\AA \subseteq \FF} y_\AA \sum_{i \in \XX- \AA} \alpha^\AA(i).
\end{equation}

Note that in any iteration of the algorithm except the last one, adding the next set $i$ to the current sets in $\AA$ did not cause the value of the knapsack to become at least $d$; that is, $\alpha(i) < d - \alpha(\AA) = d_\AA$ at that point in the algorithm. Thus, for all sets $i \in \AA$ except $l$, $\alpha^\AA(i) = \min(\alpha(i), d_\AA) = \alpha(i)$, for the point in the algorithm at which $\AA$ was the current set of sets. Thus, we can rewrite

\begin{equation}
\sum_{i \in \XX-\AA}  \alpha^\AA(i) =  \alpha^\AA(l) + \sum_{i \in \XX - \AA : i \neq l} \alpha^\AA(i) = \alpha^\AA(l) + \alpha(\XX-\{l\}) - \alpha(\AA).
\end{equation}

Note that $\alpha^\AA(l)  \leq d_\AA$ by definition, and as argued at the beginning of the proof $\alpha(\XX-\{l\}) < d$ so that $\alpha(\XX-\{l\})  - \alpha(\AA) < d - \alpha(\AA)) = d_\AA$; thus, we have that

\begin{equation}
\alpha^\AA(l) + \alpha(\XX-\{l\}) - \alpha(\AA) < 2d_\AA.
\end{equation}

Therefore,

\begin{equation}\label{2opt}
\sum_{i \in \XX} w(i) = \sum_{\AA \subseteq \FF} y_\AA \sum_{i \in \XX- \AA} \alpha^\AA(i)< 2 \sum_{A : A \subseteq \FF} d_\AA y_\AA  \leq 2 \text{\opt},
\end{equation}

where the final inequality follows by weak duality since $\sum_{A : A \subseteq \FF} d_\AA y_\AA + \sum_{j\in[n]}y_j$ is the dual objective function.

Note that our algorithm also returns $\sum_{i\in \mathcal{A}^\prime - \mathcal{X}} w(i)x_i $. It is interesting to see that our algorithm picks $\AA^\pr-\XX$ sets only when \XX does not constitute a valid set cover. Therefore, given \XX, our original problem now reduces to find only a valid set cover as the desired value is already met by $\alpha(\XX)$.

We know that the primal dual algorithm for the \setc problem is a $f$ factor approximation algorithm where $f$ is the frequency of the most frequent element, see \cite{williamson2011design}. 


Therefore, from Equation \ref{2opt}, we have 
\begin{align}
    ALG &= \sum_{i\in \AA^\pr} w(i)x_i \\
        &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \AA^\pr - \XX} w(i)x_i \\
        &\leq 2 \sum_{A : A \subseteq I} d_\AA y_\AA + f\sum_{j\in[n]}y_j\\
       % &\leq max(2,f) \text{\opt} \\
       &\leq f( \sum_{A : A \subseteq I} d_\AA y_\AA + \sum_{j\in[n]}y_j)\\
        &= f\text{\opt}
\end{align}
\end{proof}



\begin{corollary}\label{hsdfactor}
Similar to Theorem \ref{thm:approxf}, we obtain a \textbf{d}-factor approximation algorithm for the \hstp problem.  
\end{corollary}


There exists a $H_g$- approximation algorithm for the \setc problem, where $g$ is the size of the maximum sized subset using the dual fitting analysis\cite{williamson2011design}. We now present an alternative approximation algorithm that returns a $H_g$ factor solution for the \setc problem using dual fitting. 


\begin{algorithm}[htb]
    \caption{A max(2, $H_g$)-algorithm for \setckp problem }
    \begin{algorithmic}[1]
        \State $y \gets 0$
        \State $\AA \gets \emptyset$
        \While{$\alpha(\AA) < d$}
             \State Increase $ y_\AA$ until for some $i \in \FF - \AA, \sum_{\BB\subseteq\FF: i \not\in \BB} \alpha^\BB(i)y_\BB \leq w(i)$
            \State $\AA \gets \AA \cup \{i\}$
        \EndWhile
        \State $\XX \gets \AA$
        \State $\UU^\pr \gets \UU-\bigcup_{i \in \XX} \SS_i $
        \State $\FF^\pr \gets \FF-\XX$
        \State $I \gets \emptyset$
        \State $\hat{S}_i \gets S_i$ for all $i \in \FF^\pr$
        \While{$I$ is not a set cover for $\UU^\pr$}
            \State $l \gets \text{arg min}_{i:\hat{S}_i \neq \emptyset} \frac{w(i)}{|\hat{S}_i|}$
            \State $I \gets I \cup \{l\}$
            \State $\hat{S}_i \gets \hat{S}_i - S_l$ for all $i\in \FF^\pr$
        \EndWhile
        \State \textbf{return} $\XX \cup \II$
    \end{algorithmic}
    \label{lognapprox}
\end{algorithm}


\begin{comment}
\begin{theorem}
    There is a (2+$H_n$) factor approximation algorithm for the \setckp problem.
\end{theorem}
\begin{proof}
Consider the Algorithm \ref{lognapprox}. Suppose our algorithm returns
\begin{align}
    ALG  &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \II} w(i)x_i 
\end{align}
From Equation \ref{2opt}, we know that $\sum_{i\in \XX} w(i)x_i$ is at most $2 \text{ Dual \opt} \leq 2 \opt$. Also, from Observation \ref{obs:hnfactor}, we have $ \sum_{i\in \II} w(i)x_i $ is at most $H_n$. Therefore, 
\begin{align}
    ALG  &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \II} w(i)x_i\\
    &\leq 2OPT + H_nOPT\\
    &= (2+H_n)\opt
\end{align}
\end{proof}

By careful analysis we obtain a better bound. We analysis the Algorithm \ref{lognapprox} using Dual Fitting. Let \( g \) be the maximum size of any subset
\( \SS_i \); that is, \( g = \max_i |\SS_i| \). 
\end{comment}
\begin{theorem}\label{hgapprosetcover}
Algorithm \ref{lognapprox} returns a solution indexed by $\XX \cup \II$ such that

\[\sum_{i \in \XX \cup \II} w(i) \leq \max(2, H_g) \cdot \text{\opt}.\]

\end{theorem}
\begin{proof}
To prove the theorem, we construct an infeasible dual solution $y$ such that
\begin{equation}
\sum_{i \in \II} w_i = \sum_{j=1}^n y_j.
\end{equation}
We will then show that \( y' = \frac{1}{H_g} y \) is a feasible dual solution. By the weak duality
theorem,
\begin{equation}
\sum_{i=j}^n y'_j \leq \text{LP \opt},
\end{equation}
so that
\begin{equation} \label{hg}
\sum_{i \in \II} w_i = \sum_{j=1}^n y_j = H_g \sum_{j=1}^n y'_j \leq H_g \cdot \text{\opt}.
\end{equation}
In order to construct the infeasible dual solution \( y \), suppose we choose to add subset \( \SS_i \) to our solution in iteration \( k \). Then for each \( e_j \in \hat{\SS}_i \), we set \( y_j = \frac{w(i)}{|\hat{\SS}_i|} \). Since each \( e_j \in \hat{\SS}_i \) is uncovered in iteration \( k \), and is then covered for the remaining iterations of the algorithm (because we added subset \( \SS_i \) to the solution), the dual variable \( y_j \) is set to a value exactly once; in particular, it is set in the iteration in which element \( e_j \) is covered. Furthermore,
\begin{equation}
w(i) = \sum_{i: e_j \in \hat{\SS}_i} y_j
\end{equation}
i,e, the weight of the subset \( \SS_i \) chosen in the \( k \)-th iteration is equal to
the sum of the duals \( y_j \) of the uncovered elements that are covered in the \( k \)-th iteration. This
immediately implies that
\begin{equation}
\sum_{j \in \II} w(i) = \sum_{i=1}^n y_j.
\end{equation}

It remains to prove that the dual solution \( y' = \frac{1}{H_g} y \) is feasible. We must show that for each subset \( \SS_i \),
\begin{equation}
\sum_{i: e_j \in \SS_i} y'_j \leq w(i).
\end{equation}
Pick an arbitrary subset \( \SS_i \). Let \( a_k \) be the number of elements
in this subset that are still uncovered at the beginning of the \( k \)-th iteration, so that \( a_1 = |\SS_i| \),
and \( a_{l+1} = 0 \). Let \( A_k \) be the uncovered elements of \( \SS_i \) covered in the \( k \)-th iteration, so that
\(|A_k| = a_k - a_{k+1}\). If subset \( \SS_p \) is chosen in the \( k \)-th iteration, then for each element \( e_j \in A_k \)
covered in the \( k \)-th iteration,
\begin{equation}
y'_j = \frac{w_p}{H_g |\hat{\SS}_p|} \leq \frac{w(i)}{H_g a_k},
\end{equation}
where \( \hat{\SS}_p \) is the set of uncovered elements of \( \SS_p \) at the beginning of the \( k \)-th iteration. The inequality follows because if \( S_p \) is chosen in the \( k \)-th iteration, it must minimize the ratio of its
weight to the number of uncovered elements it contains. Thus,
\begin{align*}
\sum_{i: e_j \in \SS_i} y'_j &= \sum_{k=1}^l \sum_{i: e_j \in A_k} y'_j \\
&\leq \sum_{k=1}^l (a_k - a_{k+1}) \frac{w(i)}{H_g a_k} \\
&\leq \frac{w(i)}{H_g} \sum_{k=1}^l \frac{a_k - a_{k+1}}{a_k} \\
&\leq \frac{w(i)}{H_g} \sum_{k=1}^l \left( \frac{1}{a_k} + \frac{1}{a_k-1} + \cdots + \frac{1}{a_{k+1} + 1} \right) \\
&\leq \frac{w(i)}{H_g} \sum_{i=1}^{|\SS_i|} \frac{1}{i} \\
&= \frac{w(i)}{H_g} H_{|\SS_i|} \\
&\leq w(i),
\end{align*}
where the final inequality follows because \( |\SS_i| \leq g \).

Now we know, 
\begin{align}
    ALG  &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \II} w(i)x_i 
\end{align}
From Equation \ref{2opt}, we know that $\sum_{i\in \XX} w(i)x_i$ is at most $2 \sum_{A : A \subseteq \FF} d_\AA y_\AA \leq 2 \opt$. Also, from Equation \ref{hg}, we have $ \sum_{i\in \II} w(i)x_i $ is at most $H_g \cdot \sum_{j\in[n]}y_j$. Therefore, 
\begin{align}
    ALG  &= \sum_{i\in \XX} w(i)x_i + \sum_{i\in \II} w(i)x_i\\
    &\leq 2 \sum_{A : A \subseteq \FF} d_\AA y_\AA  + H_g \sum_{j\in[n]}y_j \\  
    &= \max(2, H_g) \left( \sum_{A : A \subseteq \FF} d_\AA y_\AA  + \sum_{j\in[n]}y_j \right)\\
    &= \max(2, H_g) \text{\opt}
\end{align}
\end{proof}
We obtain the following corollary from Theorem \ref{thm:approxf}.

Since \vcknapsack is a special case of the \setck problem it follows that:

\begin{corollary}\label{2factorvc}
There is a 2-approximation algorithm for the \vcktp problem.  
\end{corollary}

However, surprisingly the same cannot be said about the \setcks problem. Interestingly, \setcks problems turns out to be hard to approximate.

\begin{theorem}\label{hardnessofapprox}
For any $\rho > 1$, there does not exist a $\rho$-approximation algorithm for the \setcks problem, unless $P = NP$.
\end{theorem}
\begin{proof}
Suppose there exists a $\rho$-approximation algorithm for \setcks problem. We consider the \vc problem, which is \NPC. In the \vc problem, we are given a graph \GG(\VV, \EE) and an integer $k$, and we must decide if there exists a subset $\VV^\pr \subseteq \VV$ of size at most $k$ such that each edge $e \in \EE$ is covered by at least one vertex in $\VV^\pr$. Given an instance of the \vc problem, we can define an instance of the \setcks problem by setting the universe of elements to be the set of edges, $\UU = \{e_1, e_2, \dots, e_n\}, \forall e_j \in \EE$, the family of subsets to be the vertices that contain the edges that are incident to the corresponding vertices, $\FF = \{v_1, v_2, \dots, v_n\}, \forall v_i \in \VV$, where each $v_i = \{ e_j \in \EE : e_j \text{ is incident on } v_i \}$. We set the weight and value of each $v_i$ to be 1 $\forall v_i \in \FF$: there exists a vertex cover of size $k$ if and only if the optimal value for this \setcks instance is $k$. Furthermore, any $\rho$ approximation algorithm must always produce a solution $\leq \rho k$ if such a solution exists. Therefore, we can answer the decision version of the \vc problem in polynomial time contradicting the assumption that $P \neq NP$.
\end{proof}

Similar results hold for the dual problem:

\begin{corollary}\label{hoa:dhs}
For any $\rho > 1$, there does not exist a $\rho$-approximation algorithm for the \hsmb problem, unless $P = NP$.
\end{corollary}

It is easy to see that vertex cover is a 2-HITTING SET problem and follows that:

\begin{corollary}\label{vc-no-poly-approx}
For any $\rho > 1$, there does not exist a $\rho$-approximation algorithm for the \vckmb problem, unless $P = NP$.
\end{corollary}

At this point, we revisit the \minimalvcknapsack problem. Interestingly, it turns out that both the versions: target value and budgeted weight are hard to approximate. To see this, let us first consider the \minimalvcknapsack problem with target value. Consider the value and weight associated with each vertex to be 1 and set the the target value $d = k$. Solving this problem is equivalent to answer the question if there exists a \minimumvcknapsack of size $k$. Thus, by adjusting the value of $k$ from 1 to $n$, we can have an answer for the minimum \vc problem in polynomial time, contradicting the assumption $\Pb \neq \NP$. Similar to Theorem \ref{hardnessofapprox}, \minimalvcknapsack problem with budgeted weight is also hard to approximate. 

\begin{theorem}\label{minimalvcknapssackhoa}
The \minimalvcknapsack problem with target value and the \minimalvcknapsack problem with budgeted weight do not admit a polynomial time $\rho$-approximation algorithm for any $\rho > 1$, unless $\Pb = \NP.$.
\end{theorem}

However, we do not rule out the possibility of a fixed parameter tractable (\FPT) algorithm. In the next section, we give a \FPT algorithm for the \minimalvcknapsack problem on graphs with bounded treewidth.  



%***********************************************************************************************************************************************************************************
\section{Results: Parameterized Complexity}
\label{parameterized}
In this section, we design a dynamic programming algorithm for the \minimalvcknapsack problem, parameterized by the \textit{treewidth} of the input graph. There exists $2^{\tw}\cdot \tw^{\OO(1)}\cdot n$ algorithm for the \vc problem \cite{cygan2015parameterized}. Using a similar approach we can have dynamic programming algorithms for the \vcknapsack and \minimumvcknapsack.

\begin{theorem}\label{vckparameterzied}
  There is an algorithm for \vcknapsack with running time $2^{\tw + 1}\cdot n\cdot {\sf min}\{s^2,d^2\}$ where $n$ is the number of vertices in the input graph, $\tw$ is the treewidth of the input graph, $s$ is the input size of the knapsack and $d$ is the input target value.   
\end{theorem} 

\begin{proof}[Proof Sketch]
Let $(G = (V_G,E_G),{(w(u))_{u \in V_G}, (\alpha(u))_{u\in V_G}}, s,d)$ be an input instance of Vertex Cover Knapsack such that $\tw=tw(G)$. We consider a nice tree decomposition $(\mathbb{T} = (V_{\mathbb{T}},E_{\mathbb{T}}),\mathcal{X})$ of $G$ that is rooted at a node $r$. 

We define a function $\ell: V_{\mathbb{T}} \rightarrow \mathbb{N}$.
%For the root $r$, $\ell(r) = 0$. 
For a vertex $t \in V_\mathbb{T}$, $\ell(t) = \sf{dist}_\mathbb{T}(t,r)$, where $r$ is the root. Note that this implies that $\ell(r) = 0$. Let us assume that the values that $\ell$ takes over the nodes of $\mathbb{T}$ is between $0$ and $L$. Now, we describe a dynamic programming algorithm over $(\mathbb{T},\mathcal{X})$ for Vertex Cover Knapsack .


%%%%%%%%
    \textbf{States:} We maintain a DP table $D$ where a state has the following components:
    \begin{enumerate}
    \item $t$ represents a node in $V_\mathbb{T}$.
    \item $\mathbb{S}$ represents a subset of the vertex subset $X_t$
    \end{enumerate}
%%%%%%
    \textbf{Interpretation of States}: For each node $t \in \mathbb{T}$ we keep a list $D[t,\mathbb{S}]$ for each $\mathbb{S} \subseteq X_t$, holding the vertex cover knapsack $\mathbb{S}'$ of $G_v$ with $\mathbb{S}' \cap X_t = \mathbb{S}$ if such a $\mathbb{S}'$ exist, and $D[t,\mathbb{S}] = \infty$ otherwise.


For each state $[t,\mathbb{S}]$, we initialize $D[t,\mathbb{S}]$ to the list $\{(0,0)\}$. Our computation shall be such that in the end each $D[t,\mathbb{S}]$ stores the set of all undominated feasible pairs $(w,\alpha)$ for the state $[t,\mathbb{S}]$.

%%%%%%
    \textbf{Dynamic Programming on $D$}: We describe the following procedure to update the table $D$. We start updating the table for states with nodes $t\in V_\mathbb{T}$ such that $\ell(t)=L$. When all such states are updated, then we move to update states where the node $t$ has $\ell(t) = L-1$, and so on till we finally update states with $r$ as the node --- note that $\ell(r) =0$. For a particular $j$, $0\leq j< L$ and a state $[t,\mathbb{S}]$ such that $\ell(t) = j$, we can assume that $D[t',\mathbb{S}']$ have been evaluated for all $t'$ such that $\ell(t')>j$ and all subsets $\mathbb{S}'$ of $X_{t'}$. Now we consider several cases by which $D[t,\mathbb{S}]$ is updated based on the nature of $t$ in $\mathbb{T}$:
    
    \begin{enumerate}
    \item Suppose $t$ is a leaf node with $X_{t} = \{v\}$ . Then $D[t,\{v\}]$ = $(w(v), \alpha(v))$ and $D[t,\phi]$ stores the pair $(0,0)$.

    \item Suppose $t$ is an introduce node. Then it has an only child $t'$ where $X_{t'} \subset X_{t}$ and there is exactly one vertex $u$ that belongs to $X_{t}$ but not $X_{t'}$. Then for all $\mathbb{S} \subseteq X_t$: First, suppose $\mathbb{S}$ is not a vertex cover of $G[X_t]$, we set $D[t,\mathbb{S}] = \infty$. \\
    Next, suppose $u \in \mathbb{S}$. Then for each pair $(w,\alpha)$ in $D[t',\mathbb{S} \setminus \{u\}]$, if $w + w(u) \leq s$ we add $(w+w(u),\alpha+\alpha(u))$ to the set in $D[t,\mathbb{S}]$. Otherwise we copy all pairs of $D[t',\mathbb{S}]$ to $D[t,\mathbb{S}]$. 
    
    \item Suppose $t$ is a forget vertex node. Then it has an only child $t'$ where $X_t \subset X_{t'}$ and there is exactly one vertex $u$ that belongs to $X_{t'}$ but not to $X_t$. Then for all $\mathbb{S} \subseteq X_t$, we copy all feasible undominated pairs stored in $D[t',\mathbb{S}]$ to $D[t,\mathbb{S}]$. If any pair stored in $D[t,\mathbb{S}]$ is dominated by any pair of $D[t',\mathbb{S} \cup \{u\}]$, we copy only the undominated pairs to $D[t,\mathbb{S}]$.
    %$D[t,\mathbb{S}]$ = min\{$D[t',\mathbb{S}]$, $D[t',\mathbb{S} \cup \{u\}]$\} \\  
  
    \item Suppose $t$ is a join node. Then it has two children $t_1,t_2$ such that $X_t = X_{t_1} = X_{t_2}$. Then for all $\mathbb{S} \subseteq X_t$, let $(w_{\mathbb{S}}, \alpha_{\mathbb{S}})$ be the total weight and value of the vertices in $\mathbb{S}$. Consider a pair $(w_1,\alpha_1)$ in $D[t_1,\mathbb{S}]$ and a pair $(w_2,\alpha_2)$ in $D[t_2,\mathbb{S}]$. Suppose $w_1 + w_2 - w_{\mathbb{S}} \leq s$. Then we add $(w_1 + w_2 - w_{\mathbb{S}}, \alpha_1+\alpha_2-\alpha_{\mathbb{S}})$ to $D[t,\mathbb{S}]$.
    \end{enumerate}
    
Finally, in the last step of updating $D[t,\mathbb{S}]$, we go through the list saved in $D[t,\mathbb{S}]$ and only keep undominated pairs.

\textbf{Running time}: There are $n$ choices for the fixed vertex $v$. Upon fixing $v$ and adding it to each bag of $(\mathbb{T}, \mathcal{X})$ we consider the total possible number of states. Observe that the number of subproblems is small: for every node $t$, we have only $2^{|X_t|}$ choices of $S$. Also, we do not need to remember $\mathbb{S}$ explicitly; remembering the undominated and feasible weight and profit pair will suffice. For each state, for each $w$ there can be at most one pair with $w$ as the first coordinate; similarly, for each $\alpha$ there can be at most one pair with $\alpha$ as the second coordinate. Thus, the number of undominated pairs in each $D[t,\mathbb{S}]$ is at most ${\sf min}\{s^2,d^2\}$ time. Since the given graph \GG has a bounded treewidth of at most $tw$, it is possible to construct a data structure in time $tw^{\OO(1)} \cdot n$ that allows performing adjacency queries in time $\OO(tw)$.  For each node $t$ it takes time $ 2^{tw} \cdot tw^{\OO(1)} \cdot {\sf min}\{s^2,d^2\}$ to compute all the values $D[t,\mathbb{S}]$. Since we can assume that the number of nodes of the given tree decompositions is $\OO(tw \cdot n)$, the total running time of the algorithm is $2^{\OO(\tw)}\cdot n\cdot {\sf min}\{s^2,d^2\}$ where $n$ is the number of vertices in the input graph, $\tw$ is the treewidth of the input graph, $s$ is the input size of the knapsack and $d$ is the input target value.

\end{proof}

The maximum allowed value for $tw$ is $n$, as we cannot have treewidth greater than the size of the nodes i.e $n$. With the above algorithm, we have a pseudo-polynomial time algorithm for trees since treewidth = 1. The following corollary holds for trees.

\begin{corollary}\label{tree-pseudo-poly}
There is an algorithm for \vcknapsackbudget for trees with complexity $\OO(n^2\cdot min\{s^2, (\alpha(\VV))^2\})$.   
\end{corollary}

We can suitably modify the algorithm for \vcknapsack to obtain an algorithm for \minimumvcknapsack. Here we keep track of each $i \in [n]$ i.e. we check if there exists a valid vertex cover of size $i$. Thus, the number of states is bounded in \FPT of $n$. We obtain the following theorem:
 
\begin{theorem}\label{minvckparameterzied}
  There is an algorithm for \minimumvcknapsack with running time $4^{\OO(\tw)}\cdot n\cdot {\sf min}\{s^2,d^2\}$ where $n$ is the number of vertices in the input graph, $\tw$ is the treewidth of the input graph, $s$ is the input size of the knapsack and $d$ is the input target value.   
 \end{theorem}

Interestingly, the same standard approach does not seem to hold good for the \minimalvcknapsack. This is so because in case of a join node, say $t$, there can exist a vertex in the solution that is not redundant in either of the subgraphs rooted at $t_1$ and $t_2$, where $t_1$ and $t_2$ are the children of $t$, but it becomes redundant for the subgraph rooted at $t$. We discuss an algorithm for \minimalvcknapsack next.

\begin{theorem} \label{fptminimal}
    There is an algorithm for \minimalvcknapsack with running time $8^{\tw + 1}\cdot n\cdot {\sf min}\{s^2,d^2\}$ where $n$ is the number of vertices in the input graph, $\tw$ is the treewidth of the input graph, $s$ is the input size of the knapsack and $d$ is the input target value.
\end{theorem}
%In this section, we design a parameterized algorithm to solve the \minimalvcknapsack problem for graphs with bounded treewidth. We denote the treewidth of a graph $G$ as $tw(G)$.

\begin{proof}
Let $(G = (V_G,E_G),{(w(u))_{u \in V_G}, (\alpha(u))_{u\in V_G}}, s,d)$ be an input instance of Minimal Vertex Cover Knapsack such that $\tw=tw(G)$. We consider a nice tree decomposition $(\mathbb{T} = (V_{\mathbb{T}},E_{\mathbb{T}}),\mathcal{X})$ of $G$ that is rooted at a node $r$. 

We define a function $\ell: V_{\mathbb{T}} \rightarrow \mathbb{N}$.
%For the root $r$, $\ell(r) = 0$. 
For a vertex $t \in V_\mathbb{T}$, $\ell(t) = \sf{dist}_\mathbb{T}(t,r)$, where $r$ is the root. Note that this implies that $\ell(r) = 0$. Let us assume that the values that $\ell$ takes over the nodes of $\mathbb{T}$ is between $0$ and $L$. Now, we describe a dynamic programming algorithm over $(\mathbb{T},\mathcal{X})$ for \minimalvcknapsack .

\begin{comment}
\subsection{Assumptions}
\begin{enumerate}
    \item Define the subgraph rooted at a node $t$ in $\mathbb{T}$ as $G_t$.
    \item Let $\mathbb{S}'$ be the minimal vertex cover of $G_t$.
    \item We denote the intersection of $\mathbb{S}'$ with $X_t$ as $\mathbb{S}$ i.e. $\mathbb{S}' \cap X_t = \mathbb{S}$.
    \item To keep track of the non redundant vertices for the graph $G_{t}$, we consider two sets $V_1$ and $V_2$ such that $V_1 \cup V_2 = \mathbb{S}$.
    \item We guess a subset $V_1$ that consists of the non redundant vertices that cover some unique edge in $G_{t}$ as the intersection of $\mathbb{S}'$ with $G_t \setminus$ the edges incident on $V_2 - V_1$.
    \item We have $2^{tw+1}$ such possibilities of $V_1$. Given $V_1$, we can obtain $V_2$. Thus, there are $2^{4(tw+1)}$ DP entries for each node $t$.
\end{enumerate}
\end{comment}
%%%%%%%%
    \textbf{States:} We maintain a DP table $D$ where a state has the following components:
    \begin{enumerate}
    \item $t$ represents a node in $V_\mathbb{T}$.
    \item $V_1$, $V_2$ are subsets of the bag $X_t$, not necessarily disjoint.
    \item $V_1$ represents the intersection of $X_t$ with the minimal vertex cover knapsack of the subgraph $G_t \setminus$ the edges incident on $V_2 \setminus V_1$.
    \end{enumerate}
%%%%%%
    \textbf{Interpretation of States:} For each node $t \in \mathbb{T}$ we keep a list $D[t,V_1,V_2]$ for each $\mathbb{S} \subseteq X_t$, holding the minimal vertex cover knapsack $\mathbb{S}'$ of $G_t$ with $\mathbb{S}' \cap X_t = \mathbb{S} = V_1 \cup V_2$, if such a $\mathbb{S}'$ exist, and $D[t,V_1,V_2] = (\infty, \infty) $ otherwise. For a node $t$, $V_1$ is the intersection of $X_t$ with the minimal vertex cover knapsack of the subgraph $G_t \setminus$ the edges incident on $V_2 \setminus V_1$.

    \textbf{Genesis of the subsets $V_1$ and $V_2$:}
    We wish to capture the information about the minimal solution in the subgraph defined by removing the edges incident on $V_2 \setminus V_1$.
    Maintaining this information at every node is essential to compute the minimal solution, especially in case of a join node. Consider that a node $t$ is a join node i.e. it has two children $t_1$ and $t_2$ such that $X_t = X_{t_1} = X_{t_2}$. The nodes $t_1$ and $t_2$ are the root nodes for the subgraphs $G_{t_1}$ and $G_{t_2}$. Here we guess a subset of vertices $\mathbb{S} \subseteq X_t$. In this case, it may so happen that all vertices in $\mathbb{S}$ might not be non-redundant. To see this, let us consider the graph $G_{t_1}$ and observe how the vertices in $\mathbb{S}$ could be redundant in $G_{t_1}$. Define $V_1'$ as the intersection of the minimal solution $\mathbb{S}'$ with graph $G_{t_1}\setminus X_{t_1}$. Similarly, call $V_2'$ as the intersection of the minimal solution $\mathbb{S}'$ with graph $G_{t_2}\setminus X_{t_2}$. Consider a vertex $a \in V_1'$, $b \in V_2$ and $c \in G_{t_2} \setminus (X_{t_2} \cup V_2')$. Now it is easy to see that the vertex $b \in V_2$ is redundant in the subgraph $G_{t_1}$. However, it is not redundant with respect to $G_{t_2}$. To keep track of non redundant vertices, we require to compute the intersection of a minimal solution in each subgraph of $G_{t_1}$, i.e we assume two subsets $W_1$ and $W_2$ of $V_1$ and maintain $W_1$ in $G_{t_1}$ such that it contains all non redundant vertices of the minimal solution in the subgraph $G_{t_1} \setminus$ edges incident on $(W_2 \cap V_2) \setminus W_1$. In a similar fashion, $W_2$ stores all the non redundant vertices of the minimal solution in the subgraph $G_{t_2} \setminus$ edges incident on $(W_1 \cup V_2) \setminus W_1$. In other words, in particular for the case of a join node $t$, for a given pair of subsets $V_1$ and $V_2$, $V_1$ is the intersection of $X_t$ with a minimal solution. The set $V_1$ is further sub divided into sets $W_1$ and $W_2$ such that $W_1$ stores the non redundant vertices of the minimal solution in the graph $G_{t_1}$. We find $W_1 \subseteq V_1$, by checking whether the removal a vertex in $V_1$, can still form a vertex cover of $G_{t_1}$, if so then we place that vertex in $W_2$. Thus, we check for all such vertices and place only the non redundant vertices in $W_1$ for the subgraph $G_{t_1}$. Similarly,we compute the non redundant vertices of $G_{t_2}$, in $W_2$. Now we can now easily compute the non redundant minimal vertex cover knapsack entries for $D[t,V_1,V_2]$ i.e.in $t_1$, the state $D[t_1, W1, W2 \cup V2]$ has to be looked up and in $t_2$, $D[t_2, W2, W1 \cup V2]$ has to be looked up. 


For each state $D[t,V_1,V_2]$, we initialize $D[t,V_1,V_2]$ to the list $\{(0,0)\}$. Our computation shall be such that in the end each $D[t,V_1,V_2]$ stores the set of all undominated feasible pairs $(w,\alpha)$ for the state $[t,V_1,V_2]$.

%%%%%%
    \textbf{Dynamic Programming on $D$:} We describe the following procedure to update the table $D$. We start updating the table for states with nodes $t\in V_\mathbb{T}$ such that $\ell(t)=L$. When all such states are updated, then we move to update states where the node $t$ has $\ell(t) = L-1$, and so on till we finally update states with $r$ as the node --- note that $\ell(r) =0$. For a particular $j$, $0\leq j< L$ and a state $[t,V_1,V_2]$ such that $\ell(t) = j$, we can assume that $D[t,V_1,V_2]$ have been evaluated for all $t'$, such that $\ell(t')>j$ and all subsets $\mathbb{S}'$ of $X_{t'}$. Now we consider several cases by which $D[t,V_1,V_2]$ is updated based on the nature of $t$ in $\mathbb{T}$:
    
    \begin{enumerate}
    \item Suppose $t$ is a leaf node with $X_{t} = \{v\}$ . Then $D[t,v,\emptyset]$ = $(w(v), \alpha(v))$, or $D[t,\emptyset,v]$ = $(0,0)$ and $D[t,\emptyset, \emptyset]$ stores the pair $(0,0)$.

    \item Suppose $t$ is an introduce node. Then it has an only child $t'$ where $X_{t'} \subset X_{t}$ and there is exactly one vertex $u$ that belongs to $X_{t}$ but not $X_{t'}$. Then for all $\mathbb{S} \subseteq X_t$: First, suppose $\mathbb{S}$ is not a vertex cover of $G[X_t]$, we set $D[t,V_1,V_2] = (\infty, \infty)$. \\
    Otherwise, we have three cases:
    \begin{enumerate}
        \item Case 1: If $u \not\in V_1 \cup V_2$, then we copy each pair $(w, \alpha)$ from $D[t',V_1,V_2]$
        \item Case 2: If $u \in V_1$, then 
        \begin{enumerate}
            \item we check if $ N(u) \setminus V_1 \ne \emptyset$, then
        
            \begin{enumerate}
                \item if for each pair $(w, \alpha)$ in $D[t',V_1 \setminus \{v\},V_2]$, $w + w(u) \leq s$, then add all such pairs $(w + w(u), \alpha +\alpha(u)$ in $D[t',V_1 \setminus \{v\},V_2]$ to $D[t,V_1,V_2]$.
                \item otherwise copy each pair $(w, \alpha)$ from $D[t',V_1 \setminus \{v\},V_2]$ to $D[t,V_1,V_2]$.
            \end{enumerate}

            \item Otherwise we store $(\infty, \infty)$.
        \end{enumerate}
        \item Case 3: $u \in V_2$, then for each pair $(w,\alpha)$ in $D[t',V_1, V_2 \setminus \{u\}]$, we copy each pair of $D[t',V_1, V_2 \setminus \{u\}]$ to $D[t,V_1,V_2]$. 
    \end{enumerate}
    
    
    \item Suppose $t$ is a forget vertex node. Then it has an only child $t'$ where $X_t \subset X_{t'}$ and there is exactly one vertex $u$ that belongs to $X_{t'}$ but not to $X_t$. We copy each undominated $(w,\alpha)$ pair stored in $D[t',V_1 \cup \{v\}, V_2]$, $D[t',V_1, V_2 \cup \{v\}]$ and $D[t',V_1 , V_2]$ to $D[t,V_1 , V_2]$.
  
    \item Suppose $t$ is a join node. Then it has two children $t_1,t_2$ such that $X_t = X_{t_1} = X_{t_2}$. Let $(w(V_1 \cap V_2), \alpha(V_1 \cap V_2))$ be the total weight and value of the vertices in $V_1 \cap V_2$. Then for all $W_1, W_2 \subseteq V_1 \subseteq X_t$, consider a pair $(w_1,\alpha_1)$ in $D[t_1,W_1, W_2 \cup V_2]$ and a pair $(w_2,\alpha_2)$ in $D[t_2,W_2, W_1 \cup V_2]$. Suppose $w_1 + w_2 - w(V_1 \cap V_2) \leq s$. Then we add ($w_1 + w_2 - w(V_1 \cap V_2),  \alpha_1+\alpha_2-\alpha(V_1 \cap V_2)$) to $D[t,V_1, V_2]$.
    \end{enumerate}
    
Finally, in the last step of updating $D[t,V_1, V_2]$, we go through the list saved in $D[t,V_1, V_2]$ and only keep undominated pairs.

\textbf{Correctness of the algorithm:} Recall that we are looking for a solution $\mathcal{U}$ that contains the fixed vertex $v$ that belongs to all bags of the tree decomposition. In each state we maintain the invariant $V_1, V_2 \subseteq X_t$ such that $V_1 = X_t \cap$ minimal vertex cover knapsack of $G_t \setminus $ edges incident on $ V_2 \setminus V_1$. First, we show that a pair $(w,\alpha)$ belonging to $D[t,V_1, V_2]$ for a node $t \in V_\mathbb{T}$ and a subset $\mathbb{S}$ of $X_t$ corresponds to a minimal vertex cover knapsack $H$ in $G_t$. Recall that $X_r = \{v\}$. Thus, this implies that a pair $(w,\alpha)$ belonging to $D[r, V_1 = \{v\}, V_2 = \emptyset )]$ corresponds to a minimal vertex cover knapsack of $G$. Moreover, the output is a pair that is feasible and with the highest value. 

In order to show that a pair $(w,\alpha)$ belonging to $D[t, V_1, V_2]$ for a node $t \in V_\mathbb{T}$ and a subset $V_1$ of $X_t$ corresponds to a minimal vertex cover knapsack of $G_t \setminus $ edges incident on $ V_2 \setminus V_1$, we need to consider the cases of what $t$ can be:


\begin{enumerate}

    \item \textbf{Leaf node}: Recall that in our modified nice tree decomposition we have added a vertex $v$ to all the bags. Suppose a leaf node $t$ contains a single vertex $v$, $D[t,v,\emptyset] = (w(v),\alpha(v))$, $D[t,\emptyset,v] = (0,0)$ and $D[L,\emptyset, \emptyset]$ stores the pair $(0, 0)$. This is true in particular when $j = L$, the base case. From now we can assume that for a node $t$ with $\ell(t) = j < L$ and all subsets $V_1, V_2 \subseteq X_t$, $D[t',V_1^{\pr\pr},V_2^{\pr\pr}]$ entries are correct and correspond to minimal vertex cover in $G_{t'} \setminus $ edges incident on $ V_2^{\pr\pr} \setminus V_1^{\pr\pr}$. when $\ell(t') > j$.

    \item \textbf{Introduce node}: When $t$ is an introduce node, there is a child $t'$. We are introducing a vertex $u$ and the edges associated with it in $G_t$. Since $\ell(t') > \ell(t)$, by induction hypothesis all entries in $D[t',V_1^{\pr\pr} = V_1 \setminus \{u\}, V_2^{\pr\pr} =V_2\setminus \{u\}]$, $D[t', V_1^{\pr\pr}=V_1\setminus \{u\},V_2^{\pr\pr} = V_2]$, and $D[t', V_1^{\pr\pr}= V_1,V_2^{\pr\pr} = V_2 \setminus \{u\}]$, $\forall$ $V_1^{\pr\pr} , V_2^{\pr\pr} \subseteq X_{t'}$ are already computed and feasible. We update pairs in $D[t,V_1,V_2]$ from $D[t',V_1 \setminus \{u\}, V_2]$ or $D[t',V_1,V_2 \setminus \{u\}]$ or $D[t',V_1 \setminus \{u\}, V_2 \setminus \{u\}]$  such that either $u$ is considered as part of a minimal solution in $G_{t} \setminus $ edges incident on $ V_2 \setminus V_1$ or not. 

    \item \textbf{Forget node}:  When $t$ is a forget node, there is a child $t'$. We are forgetting a vertex $u$ and the edges associated with it in $G_t$. Since $\ell(t') > \ell(t)$, by induction hypothesis all entries in $D[t',V_1^{\pr\pr} = V_1 \cup \{u\}, V_2^{\pr\pr} = V_2]$, $D[t',V_1^{\pr\pr}=V_1,V_2^{\pr\pr}=V_2 \cup \{u\}]$, and  $D[t',V_1^{\pr\pr}=V_1,V_2^{\pr\pr}=V_2]$, $\forall$ $V_1^{\pr\pr}, V_2^{\pr\pr} \subseteq X_{t'}$ are already computed and feasible. We copy each undominated $(w,\alpha)$ pair stored in $D[t',V_1 \cup \{u\}, V_2]$, $D[t',V_1, V_2 \cup \{u\}]$ and $D[t',V_1 , V_2]$ to $D[t,V_1,V_2]$.

    \item \textbf{Join node}: When $t$ is a forget node, there are two children $t_1$ and $t_2$ of $t$, such that $X_t = X_{t_1} = X_{t_2}$. For all subsets  $V_1 \subseteq X_t$ we partition $V_1$ into two subsets $W_1$ and $W_2$ (not necessarily disjoint) such that $W_1$ is the intersection of $X_{t_1}$ with minimal solution in the graph $G_{t_1} \setminus $ edges incident on $(W_2 \cup V_2) \setminus W_1$. Similarly, $W_2$ is the intersection of $X_{t_2}$ with minimal solution in the graph $G_{t_2} \setminus $ edges incident on $(W_1 \cup V_2) \setminus W_2$. By the induction hypothesis, the computed entries in $D[t_1,W_1, W_2 \cup V_2]$ and $D[t_2,W_2, W_1 \cup V_2]$ where $W_1 \cup W_2 = V_1$ are correct and store the non redundant minimal vertex cover for the subgraph $G_{t_1}$ in $W_1$ and similarly, $W_2$ for $G_{t_2}$. Now we add ($w_1 + w_2 - w(V_1 \cap V_2),  \alpha_1+\alpha_2-\alpha\{V_1 \cap V_2))$) to $D[t,V_1, V_2]$.

\end{enumerate}

What remains to be shown is that an undominated feasible solution $\mathcal{U}$ of \minimalvcknapsack in $G$ is contained in $D[r,\{v\},\emptyset]$. Let $w$ be the weight of $\mathcal{U}$ and $\alpha$ be the value. Recall that $v \in \mathcal{U}$. For each $t$, we consider the subgraph $G_t$ and observe how the minimal solution $\mathcal{S}'$ interacts with $G_t$. Let $\hat{V}_1, \hat{V}_2, \ldots, \hat{V}_m$ be components of $G_t \cap \mathcal{U}$ and let for each $1 \leq i \leq m$, $\mathcal{S}_i = X_t \cap \hat{V}_i$. Also, let $\hat{V}_0 = X_t \setminus \mathcal{U}$. Consider $\mathcal{S} = (\hat{V}_0, \hat{V}_1, \hat{V}_2, \ldots, \hat{V}_m)$. For each $\mathcal{S}_i$, we define subsets $V_1$ and $V_2$ such that $V_1, V_2 \subseteq \mathcal{S}_i$, and $V_1 \cup V_2 = \mathcal{S}_i$, $\forall i \in [m]$. The algorithm updates in $D[t,V_1,V_2]$ the pair $(w',\alpha')$ for the subsolution $(G_{t} \setminus $ edges incident on $ V_2) \cap \mathcal{U}$. Therefore, $D[r,\{v\},\emptyset]$ contains the pair $(w,\alpha)$. Thus, we are done.




\textbf{Running Time:}
There are $n$ choices for the fixed vertex $v$. Upon fixing $v$ and adding it to each bag of $(\mathbb{T}, \mathcal{X})$ we consider the total possible number of states. Observe that the number of subproblems is small: for every node $t$, we have only $2^{|X_t|}$ choices of $S$, $2^{|S|}$ choices for $V_1$ and $2^{|V_1|}$ choices for $W_1$ i,e, $\OO(8^{|X_t|})$. Also, we do not need to remember $\mathbb{S}$ explicitly; remembering the undominated and feasible weight and profit pair will suffice. Therefore, are at most $\OO(n)\cdot 8^{\tw + 1}$ states. For each state, since we are keeping only undominated pairs, for each $w$ there can be at most one pair with $w$ as the first coordinate; similarly, for each $\alpha$ there can be at most one pair with $\alpha$ as the second coordinate. Thus, the number of undominated pairs in each $D[t,V_1, V_2]$ is at most ${\sf min}\{s^2,d^2\}$. By the description of the algorithm, the maximum length of the list stored at $D[t,V_1, V_2]$ during updation, but before the check is made for only undominated pairs, is $8^{\tw + 1}\cdot{\sf min}\{s^2,d^2\}$. Thus, updating the DP table at any vertex takes $8^{\tw + 1}\cdot{\sf min}\{s^2,d^2\}$ time. Since there are $\OO(n\cdot\tw)$ vertices in $\mathbb{T}$, the total running time of the algorithm is $8^{\tw + 1}\cdot n\cdot {\sf min}\{s^2,d^2\}$. 
\end{proof}

The treewidth of a tree is 1. This implies the following corollary:

\begin{corollary}\label{thm:vckp-tree-algo}
There exists an algorithm for \vcknapsack for trees running in time $\OO( n\cdot {\sf min}\{s^2,d^2\})$.
\end{corollary}

The above corollary also implies that \vcknapsack for trees is pseudo polynomial.

\section{Conclusion}
\label{conclusion}
 We study the classical Knapsack problem with the graph theoretic constraints, namely vertex cover and its interesting variants like \minimumvcknapsack, \minimalvcknapsack and \vcknapsackbudget for both general graphs and trees. We show that the \vcknapsack is strongly \NPC and show the computational complexity of the other variants. We also discuss the generalized version of the problem i.e. \setck and \hs. Our results show the existence of a 2-factor approximation algorithm for \vcktp and the unlikeliness of a $\rho$-factor algorithm for \vckmb. Parameterized by the treewidth of a given graph, we also prove that all the variants admit \FPT algorithms.  





%%
%% Bibliography
%%

%% Please use bibtex, 
\newpage
\bibliography{references}

\appendix

\

\end{document}

